MVQA: Mamba with Unified Sampling for Efficient Video Quality Assessment

The rapid growth of long-duration, high-definition videos has made efficient video quality assessment (VQA) a critical challenge. Existing research typically tackles this problem through two main strategies: reducing model parameters and resampling inputs. However, light-weight Convolution Neural Networks (CNN) and Transformers often struggle to balance efficiency with high performance due to the requirement of long-range modeling capabilities. Recently, the state-space model, particularly Mamba, has emerged as a promising alternative, offering linear complexity with respect to sequence length. Meanwhile, efficient VQA heavily depends on resampling long sequences to minimize computational costs, yet current resampling methods are often weak in preserving essential semantic information. In this work, we present MVQA, a Mamba-based model designed for efficient VQA along with a novel Unified Semantic and Distortion Sampling (USDS) approach. USDS combines semantic patch sampling from low-resolution videos and distortion patch sampling from original-resolution videos. The former captures semantically dense regions, while the latter retains critical distortion details. To prevent computation increase from dual inputs, we propose a fusion mechanism using pre-defined masks, enabling a unified sampling strategy that captures both semantic and quality information without additional computational burden. Experiments show that the proposed MVQA, equipped with USDS, achieve comparable performance to state-of-the-art methods while being $2\times$ as fast and requiring only $1/5$ GPU memory.

==> 1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}[htbp]
	\centering
	\setlength{\abovecaptionskip}{0.1cm}
	%	\setlength{\belowcaptionskip}{-0.1cm}
	%	
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{img//1.1.png}
		\centerline{ \footnotesize (a) GPU Memory Comparison}
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{img//1.2.png}
		\centerline{\footnotesize (b) Speed Comparison}
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{img//1.3.png}
		\centerline{\footnotesize (c) GPU Memory Comparison}
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{img//1.4.png}
		\centerline{\footnotesize (d) Accuracy Comparison}
	\end{minipage}
	
	\caption{Performance and efficiency comparisons between FAST-VQA\cite{paper29} and our MVQA-tiny. Our method achieves comparable results while running up to $2\times$ faster than the current most efficient FAST-VQA, and reducing GPU memory usage by $5.3\times$. This advantage further scales with increased video frames and batch size.}
	\label{fig1}
	\vspace{-0.4cm}
\end{figure}

With the widespread adoption of high-definition portable recording devices and the ongoing advancements in video compression and network technologies, ordinary users can now effortlessly capture long-duration, high-resolution videos (e.g., 2K, 4K) and upload them to online platforms.
The increasing length and size of video present substantial challenges for video quality assessment (VQA) algorithms.
Therefore, developing efficient methods to quickly evaluate massive amounts of video data to ensure a high-quality viewing experience has become a pressing challenge.

Traditional VQA methods \cite{paper7,paper8,paper9,paper10,paper11,paper12,paper13,paper14} primarily rely on handcrafted features. While these approaches are computationally efficient and have low complexity, they struggle to effectively capture the intricate, high-dimensional characteristics of videos. As a result, their performance tends to be limited when processing high-resolution videos with rich details and diverse content. 
In contrast, deep learning-based VQA methods \cite{paper41,paper15,paper42,paper16,paper17,paper18,paper29,paper23,paper43,paper19,paper45,paper46,paper20,paper68,paper69}, particularly Convolutional Neural Networks (CNNs) \cite{paper47,paper48,paper49,paper50,paper51,paper52,paper55,paper56} and Transformers \cite{paper44,paper53,paper54}, have demonstrated substantial advantages in handling complex video tasks. 
However, deep learning-based approaches typically incur high computational costs, including significant memory consumption and lengthy processing times, which become particularly challenging when dealing with large-scale, high-resolution video data. 
Specifically, although CNNs excel at extracting local features, they face limitations in modeling long-range dependencies and processing large-scale datasets. On the other hand, while Transformer models excel at capturing global dependencies, their computational complexity grows quadratically with video length and resolution, posing considerable challenges when applied to large video datasets. Consequently, relying on either CNNs or Transformers for VQA often fails to strike an effective balance between performance and computational efficiency.

%Recently, as a novel sequence modeling architecture, Mamba \cite{paper70} has attracted widespread attention for its ability to effectively solve the computational bottleneck of traditional deep learning models when dealing with long sequences. Specifically, Mamba is essentially a State Space Model (SSM) \cite{paper71,paper72,paper73,paper74,paper75,paper76} that models long-range dependencies in time-series data through a set of state transfer equations.
%Notably, the computational complexity of SSM grows linearly with the length of the input sequence. In addition to its advantages in temporal modeling, Mamba has also demonstrated outstanding performance in visual tasks \cite{paper82,paper83,paper84,paper85,paper86,paper87}, suggesting that it possesses not only strong temporal modeling capabilities but also excellent spatio-temporal awareness.
%In the context of VQA, the advantages of Mamba are particularly prominent. Videos typically contain a substantial amount of redundant information, and traditional VQA methods may suffer from reduced efficiency and accuracy due to excessive computational burden. However, the linear time complexity of the Mamba-based model allows VQA systems to efficiently process large-scale video data while accurately capturing spatio-temporal relationships and semantic features. This is especially beneficial when dealing with long-duration and high-resolution videos, where Mamba significantly enhances processing efficiency while maintaining high-quality evaluation accuracy. Therefore, Mamba-based VQA methods provide a practical and effective solution for efficient and precise video quality assessment.

Mamba \cite{paper70}, a novel sequence modeling architecture, has gained attention for addressing computational bottlenecks in processing long sequences. As a State Space Model (SSM) \cite{paper71,paper72,paper73,paper74,paper75,paper76}, Mamba models long-range dependencies with state transfer equations and linear complexity relative to input length. Beyond temporal modeling, Mamba also excels in spatio-temporal tasks \cite{paper82,paper83,paper84,paper85,paper86,paper87}, making it particularly advantageous for VQA. Traditional VQA models often struggle with redundant video data and high computational demands, but Mamba’s efficiency allows it to handle large-scale video data accurately and with reduced processing time, especially for long and high-resolution videos. Thus, Mamba-based VQA offers a practical solution for efficient and precise video quality assessment.


Moreover, the computational complexity and accuracy of VQA models are influenced not only by the model architecture but also by the sampling strategy employed. 
Traditional sampling methods like cropping \cite{paper77,paper78} and resizing \cite{paper79} reduce computational load but often distort video quality. To better retain quality information, Wu et al. \cite{paper29} introduced Grid Mini-patch Sampling (GMS), which samples small patches across uniform grids to preserve quality and temporal features. However, the fragmentation from grid sampling limits semantic information capture, which is essential for VQA accuracy \cite{paper21,paper15,paper22,paper23,paper80,paper81}. Thus, an effective sampling strategy should maintain both video quality and semantic information.
%
%
%Traditional sampling techniques, such as cropping \cite{paper77,paper78} and resizing \cite{paper79}, while effective in reducing computational overhead, often introduce significant distortions to the video quality, which in turn can negatively impact model performance.
%To effectively preserve the quality information of the original video after sampling, Wu et al. \cite{paper29} proposed Grid Mini-patch Sampling (GMS), which samples small patches from uniformly divided grids within the video frames to retain certain quality and temporal features. While this method effectively preserves video quality information, the fragmentation introduced by grid sampling makes it difficult to capture the semantic information of the video effectively. 
%However, some studies \cite{paper21,paper15,paper22,paper23,paper80,paper81} have shown that semantic information plays a crucial role in VQA, as it provides richer contextual insights, particularly when assessing video quality. Therefore, to more accurately evaluate video quality, the sampling strategy should not only comprehensively reflect the quality characteristics of the video but also retain as much of the semantic information as possible.
%
%VQA model performance depends on both architecture and sampling strategy. Traditional sampling methods like cropping \cite{paper77,paper78} and resizing \cite{paper79} reduce computational load but often distort video quality. To better retain quality information, Wu et al. \cite{paper29} introduced Grid Mini-patch Sampling (GMS), which samples small patches across uniform grids to preserve quality and temporal features. However, the fragmentation from grid sampling limits semantic information capture, which is essential for VQA accuracy \cite{paper21,paper15,paper22,paper23,paper80,paper81}. Thus, an effective sampling strategy should maintain both video quality and semantic information.

\begin{figure}[t]
	\centering
	\setlength{\abovecaptionskip}{0.1cm}
	\includegraphics[scale=0.07]{img//1.5.png}
	\caption{Comparison of semantic information retained by USDS with different samples (resize, Fragments \cite{paper29}).}
	\label{fig1.5}
	\vspace{-0.4cm}
\end{figure}


Based on the above analysis, we propose Unified Semantic and Distortion Sampling (USDS), which not only effectively samples video distortions but also preserves the semantic information of the video.
As shown in \cref{fig1.5}, we use CLIP \cite{paper24}, with its strong zero-shot prediction capabilities, to verify that USDS effectively preserves semantic information.
Specifically, USDS first obtains a downsampled version to capture the semantic information of the video, then performs grid sampling to capture the distortion information. These two sampled maps are then combined at a specified ratio through masking.  Additionally, we introduce MVQA, a VQA model fully based on state space models, and experiments demonstrate that our model achieves a balance between performance and efficiency. As shown in \cref{fig1}, Compared to the current most efficient model, FastVQA, our MVQA-tiny achieves comparable performance while offering faster computation speed and lower memory usage.

Our contributions can be summarized as follows:
\begin{itemize}
	%	\item To the best of our knowledge, this work is the first attempt to apply state-space models in the VQA domain.
	%	\item We propose a novel sampling method, USDS, which introduces semantic information through masking fusion applied to distortion sampling. This approach overcomes the limitations of previous methods that could not account for both video distortion and semantic simultaneously.
	%%	A novel sampling method, USDS, is proposed, which introduces semantic information through masking fusion on top of distortion sampling. This approach addresses the limitation of previous sampling methods, which failed to simultaneously account for both video distortion and semantic content.
	%	\item We propose the first Mamba-based VQA model, MVQA, which effectively balances computational efficiency and modeling capacity.
	%	\item Extensive experiments show that MVQA surpasses state-of-the-art methods while ensuring efficient computation and smaller memory usage.
	\item To the best of our knowledge, this is the first work to successfully apply state-space models in the VQA domain, which effectively balances computational efficiency and performance. 
	\item We propose a novel sampling method, USDS, which unifies semantic and distortion patch sampling through masked fusion. This approach addresses the limitation of previous sampling methods, which failed to simultaneously account for both semantic content and distortions.
	\item We conduct extensive experiments to demonstrate that MVQA outperforms both transformer-based and CNN-based methods, while ensuring efficient computation and smaller memory usage.
	
\end{itemize}



%
%Traditional VQA methods mainly rely on hand-designed features, and while these methods have low computational complexity and high efficiency, they tend to have limited performance in dealing with high-resolution videos with rich details and diverse contents because they cannot effectively capture complex and high-dimensional features in videos.Comparatively, deep learning-based VQA methods, especially Convolutional Neural Networks (CNNs) and Transformer, show significant advantages in processing complex video tasks.Nonetheless, deep learning-based methods usually require high computational overheads, including huge memory consumption and long computational processes, which is particularly prominent when dealing with large-scale, high-resolution video data.
%Specifically, while CNNs can effectively extract local features, they have limitations in modeling long-range dependencies and handling large-scale datasets; while Transformer models, while they have advantages in capturing global dependencies, their computational complexity grows quadratically with the increase of video length and resolution, leading to greater challenges when applied on large-scale video datasets. Therefore, relying solely on CNN or Transformer for VQA often fails to guarantee performance while effectively controlling computational complexity.


%With the widespread use of high-definition portable devices and advances in video compression and network technologies, users can easily capture and upload long-duration, high-resolution (2K, 4K) videos. However, issues such as blur, noise, and color degradation often arise during acquisition, transmission, and processing, significantly affecting video quality. The increasing length and size of videos pose significant challenges for quality assessment algorithms. Therefore, developing efficient methods to rapidly evaluate large volumes of video data and ensure a high-quality viewing experience has become an urgent challenge.






==> ICCV2025-Author-Kit-Feb/0_abstract.tex <==
\begin{abstract}
	
The rapid growth of long-duration, high-definition videos has made efficient video quality assessment (VQA) a critical challenge.
Existing research typically tackles this problem through two main strategies: reducing model parameters and resampling inputs.
However, light-weight Convolution Neural Networks (CNN) and Transformers often struggle to balance efficiency with high performance due to the requirement of long-range modeling capabilities. 
Recently, the state-space model, particularly Mamba, has emerged as a promising alternative, offering linear complexity with respect to sequence length. 
Meanwhile, efficient VQA heavily depends on resampling long sequences to minimize computational costs, yet current resampling methods are often weak in preserving essential semantic information.
In this work, we present MVQA, a Mamba-based model designed for efficient VQA along with a novel Unified Semantic and Distortion Sampling (USDS) approach.
USDS combines semantic patch sampling from low-resolution videos and distortion patch sampling from original-resolution videos. The former captures semantically dense regions, while the latter retains critical distortion details. 
To prevent computation increase from dual inputs, we propose a fusion mechanism using pre-defined masks, enabling a unified sampling strategy that captures both semantic and quality information without additional computational burden.
Experiments show that the proposed MVQA, equipped with USDS, achieve comparable  performance to state-of-the-art methods while being $2\times$ as fast and requiring only $1/5$ GPU memory.

\end{abstract}

==> ICCV2025-Author-Kit-Feb/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}[htbp]
	\centering
	\setlength{\abovecaptionskip}{0.1cm}
	%	\setlength{\belowcaptionskip}{-0.1cm}
	%	
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{img//1.1.png}
		\centerline{ \footnotesize (a) GPU Memory Comparison}
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{img//1.2.png}
		\centerline{\footnotesize (b) Speed Comparison}
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{img//1.3.png}
		\centerline{\footnotesize (c) GPU Memory Comparison}
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{img//1.4.png}
		\centerline{\footnotesize (d) Accuracy Comparison}
	\end{minipage}
	
	\caption{Performance and efficiency comparisons between FAST-VQA\cite{paper29} and our MVQA-tiny. Our method achieves comparable results while running up to $2\times$ faster than the current most efficient FAST-VQA, and reducing GPU memory usage by $5.3\times$. This advantage further scales with increased video frames and batch size.}
	\label{fig1}
	\vspace{-0.4cm}
\end{figure}

With the widespread adoption of high-definition portable recording devices and the ongoing advancements in video compression and network technologies, ordinary users can now effortlessly capture long-duration, high-resolution videos (e.g., 2K, 4K) and upload them to online platforms.
The increasing length and size of video present substantial challenges for video quality assessment (VQA) algorithms.
Therefore, developing efficient methods to quickly evaluate massive amounts of video data to ensure a high-quality viewing experience has become a pressing challenge.

Traditional VQA methods \cite{paper7,paper8,paper9,paper10,paper11,paper12,paper13,paper14} primarily rely on handcrafted features. While these approaches are computationally efficient and have low complexity, they struggle to effectively capture the intricate, high-dimensional characteristics of videos. As a result, their performance tends to be limited when processing high-resolution videos with rich details and diverse content. 
In contrast, deep learning-based VQA methods \cite{paper41,paper15,paper42,paper16,paper17,paper18,paper29,paper23,paper43,paper19,paper45,paper46,paper20,paper68,paper69}, particularly Convolutional Neural Networks (CNNs) \cite{paper47,paper48,paper49,paper50,paper51,paper52,paper55,paper56} and Transformers \cite{paper44,paper53,paper54}, have demonstrated substantial advantages in handling complex video tasks. 
However, deep learning-based approaches typically incur high computational costs, including significant memory consumption and lengthy processing times, which become particularly challenging when dealing with large-scale, high-resolution video data. 
Specifically, although CNNs excel at extracting local features, they face limitations in modeling long-range dependencies and processing large-scale datasets. On the other hand, while Transformer models excel at capturing global dependencies, their computational complexity grows quadratically with video length and resolution, posing considerable challenges when applied to large video datasets. Consequently, relying on either CNNs or Transformers for VQA often fails to strike an effective balance between performance and computational efficiency.

%Recently, as a novel sequence modeling architecture, Mamba \cite{paper70} has attracted widespread attention for its ability to effectively solve the computational bottleneck of traditional deep learning models when dealing with long sequences. Specifically, Mamba is essentially a State Space Model (SSM) \cite{paper71,paper72,paper73,paper74,paper75,paper76} that models long-range dependencies in time-series data through a set of state transfer equations.
%Notably, the computational complexity of SSM grows linearly with the length of the input sequence. In addition to its advantages in temporal modeling, Mamba has also demonstrated outstanding performance in visual tasks \cite{paper82,paper83,paper84,paper85,paper86,paper87}, suggesting that it possesses not only strong temporal modeling capabilities but also excellent spatio-temporal awareness.
%In the context of VQA, the advantages of Mamba are particularly prominent. Videos typically contain a substantial amount of redundant information, and traditional VQA methods may suffer from reduced efficiency and accuracy due to excessive computational burden. However, the linear time complexity of the Mamba-based model allows VQA systems to efficiently process large-scale video data while accurately capturing spatio-temporal relationships and semantic features. This is especially beneficial when dealing with long-duration and high-resolution videos, where Mamba significantly enhances processing efficiency while maintaining high-quality evaluation accuracy. Therefore, Mamba-based VQA methods provide a practical and effective solution for efficient and precise video quality assessment.

Mamba \cite{paper70}, a novel sequence modeling architecture, has gained attention for addressing computational bottlenecks in processing long sequences. As a State Space Model (SSM) \cite{paper71,paper72,paper73,paper74,paper75,paper76}, Mamba models long-range dependencies with state transfer equations and linear complexity relative to input length. Beyond temporal modeling, Mamba also excels in spatio-temporal tasks \cite{paper82,paper83,paper84,paper85,paper86,paper87}, making it particularly advantageous for VQA. Traditional VQA models often struggle with redundant video data and high computational demands, but Mamba’s efficiency allows it to handle large-scale video data accurately and with reduced processing time, especially for long and high-resolution videos. Thus, Mamba-based VQA offers a practical solution for efficient and precise video quality assessment.


Moreover, the computational complexity and accuracy of VQA models are influenced not only by the model architecture but also by the sampling strategy employed. 
Traditional sampling methods like cropping \cite{paper77,paper78} and resizing \cite{paper79} reduce computational load but often distort video quality. To better retain quality information, Wu et al. \cite{paper29} introduced Grid Mini-patch Sampling (GMS), which samples small patches across uniform grids to preserve quality and temporal features. However, the fragmentation from grid sampling limits semantic information capture, which is essential for VQA accuracy \cite{paper21,paper15,paper22,paper23,paper80,paper81}. Thus, an effective sampling strategy should maintain both video quality and semantic information.
%
%
%Traditional sampling techniques, such as cropping \cite{paper77,paper78} and resizing \cite{paper79}, while effective in reducing computational overhead, often introduce significant distortions to the video quality, which in turn can negatively impact model performance.
%To effectively preserve the quality information of the original video after sampling, Wu et al. \cite{paper29} proposed Grid Mini-patch Sampling (GMS), which samples small patches from uniformly divided grids within the video frames to retain certain quality and temporal features. While this method effectively preserves video quality information, the fragmentation introduced by grid sampling makes it difficult to capture the semantic information of the video effectively. 
%However, some studies \cite{paper21,paper15,paper22,paper23,paper80,paper81} have shown that semantic information plays a crucial role in VQA, as it provides richer contextual insights, particularly when assessing video quality. Therefore, to more accurately evaluate video quality, the sampling strategy should not only comprehensively reflect the quality characteristics of the video but also retain as much of the semantic information as possible.
%
%VQA model performance depends on both architecture and sampling strategy. Traditional sampling methods like cropping \cite{paper77,paper78} and resizing \cite{paper79} reduce computational load but often distort video quality. To better retain quality information, Wu et al. \cite{paper29} introduced Grid Mini-patch Sampling (GMS), which samples small patches across uniform grids to preserve quality and temporal features. However, the fragmentation from grid sampling limits semantic information capture, which is essential for VQA accuracy \cite{paper21,paper15,paper22,paper23,paper80,paper81}. Thus, an effective sampling strategy should maintain both video quality and semantic information.

\begin{figure}[t]
	\centering
	\setlength{\abovecaptionskip}{0.1cm}
	\includegraphics[scale=0.07]{img//1.5.png}
	\caption{Comparison of semantic information retained by USDS with different samples (resize, Fragments \cite{paper29}).}
	\label{fig1.5}
	\vspace{-0.4cm}
\end{figure}


Based on the above analysis, we propose Unified Semantic and Distortion Sampling (USDS), which not only effectively samples video distortions but also preserves the semantic information of the video.
As shown in \cref{fig1.5}, we use CLIP \cite{paper24}, with its strong zero-shot prediction capabilities, to verify that USDS effectively preserves semantic information.
Specifically, USDS first obtains a downsampled version to capture the semantic information of the video, then performs grid sampling to capture the distortion information. These two sampled maps are then combined at a specified ratio through masking.  Additionally, we introduce MVQA, a VQA model fully based on state space models, and experiments demonstrate that our model achieves a balance between performance and efficiency. As shown in \cref{fig1}, Compared to the current most efficient model, FastVQA, our MVQA-tiny achieves comparable performance while offering faster computation speed and lower memory usage.

Our contributions can be summarized as follows:
\begin{itemize}
	%	\item To the best of our knowledge, this work is the first attempt to apply state-space models in the VQA domain.
	%	\item We propose a novel sampling method, USDS, which introduces semantic information through masking fusion applied to distortion sampling. This approach overcomes the limitations of previous methods that could not account for both video distortion and semantic simultaneously.
	%%	A novel sampling method, USDS, is proposed, which introduces semantic information through masking fusion on top of distortion sampling. This approach addresses the limitation of previous sampling methods, which failed to simultaneously account for both video distortion and semantic content.
	%	\item We propose the first Mamba-based VQA model, MVQA, which effectively balances computational efficiency and modeling capacity.
	%	\item Extensive experiments show that MVQA surpasses state-of-the-art methods while ensuring efficient computation and smaller memory usage.
	\item To the best of our knowledge, this is the first work to successfully apply state-space models in the VQA domain, which effectively balances computational efficiency and performance. 
	\item We propose a novel sampling method, USDS, which unifies semantic and distortion patch sampling through masked fusion. This approach addresses the limitation of previous sampling methods, which failed to simultaneously account for both semantic content and distortions.
	\item We conduct extensive experiments to demonstrate that MVQA outperforms both transformer-based and CNN-based methods, while ensuring efficient computation and smaller memory usage.
	
\end{itemize}



%
%Traditional VQA methods mainly rely on hand-designed features, and while these methods have low computational complexity and high efficiency, they tend to have limited performance in dealing with high-resolution videos with rich details and diverse contents because they cannot effectively capture complex and high-dimensional features in videos.Comparatively, deep learning-based VQA methods, especially Convolutional Neural Networks (CNNs) and Transformer, show significant advantages in processing complex video tasks.Nonetheless, deep learning-based methods usually require high computational overheads, including huge memory consumption and long computational processes, which is particularly prominent when dealing with large-scale, high-resolution video data.
%Specifically, while CNNs can effectively extract local features, they have limitations in modeling long-range dependencies and handling large-scale datasets; while Transformer models, while they have advantages in capturing global dependencies, their computational complexity grows quadratically with the increase of video length and resolution, leading to greater challenges when applied on large-scale video datasets. Therefore, relying solely on CNN or Transformer for VQA often fails to guarantee performance while effectively controlling computational complexity.


%With the widespread use of high-definition portable devices and advances in video compression and network technologies, users can easily capture and upload long-duration, high-resolution (2K, 4K) videos. However, issues such as blur, noise, and color degradation often arise during acquisition, transmission, and processing, significantly affecting video quality. The increasing length and size of videos pose significant challenges for quality assessment algorithms. Therefore, developing efficient methods to rapidly evaluate large volumes of video data and ensure a high-quality viewing experience has become an urgent challenge.






==> ICCV2025-Author-Kit-Feb/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}[htbp]
	\centering
	\setlength{\abovecaptionskip}{0.1cm}
	%	\setlength{\belowcaptionskip}{-0.1cm}
	%	
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{1.1.png}
		\centerline{ \footnotesize (a) GPU Memory Comparison}
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{1.2.png}
		\centerline{\footnotesize (b) Speed Comparison}
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{1.3.png}
		\centerline{\footnotesize (c) GPU Memory Comparison}
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{1.4.png}
		\centerline{\footnotesize (d) Accuracy Comparison}
	\end{minipage}
	
	\caption{Performance and efficiency comparisons between FAST-VQA\cite{paper29} and our MVQA-tiny. Our method achieves comparable results while running up to $2\times$ faster than the current most efficient FAST-VQA, and reducing GPU memory usage by $5.3\times$. This advantage further scales with increased video frames and batch size.}
	\label{fig1}
	\vspace{-0.4cm}
\end{figure}

With the widespread adoption of high-definition portable recording devices and the ongoing advancements in video compression and network technologies, ordinary users can now effortlessly capture long-duration, high-resolution videos (e.g., 2K, 4K) and upload them to online platforms.
The increasing length and size of video present substantial challenges for video quality assessment (VQA) algorithms.
Therefore, developing efficient methods to quickly evaluate massive amounts of video data to ensure a high-quality viewing experience has become a pressing challenge.

Traditional VQA methods \cite{paper7,paper8,paper9,paper10,paper11,paper12,paper13,paper14} primarily rely on handcrafted features. While these approaches are computationally efficient and have low complexity, they struggle to effectively capture the intricate, high-dimensional characteristics of videos. As a result, their performance tends to be limited when processing high-resolution videos with rich details and diverse content. 
In contrast, deep learning-based VQA methods \cite{paper41,paper15,paper42,paper16,paper17,paper18,paper29,paper23,paper43,paper19,paper45,paper46,paper20,paper68,paper69}, particularly Convolutional Neural Networks (CNNs) \cite{paper47,paper48,paper49,paper50,paper51,paper52,paper55,paper56} and Transformers \cite{paper44,paper53,paper54}, have demonstrated substantial advantages in handling complex video tasks. 
However, deep learning-based approaches typically incur high computational costs, including significant memory consumption and lengthy processing times, which become particularly challenging when dealing with large-scale, high-resolution video data. 
Specifically, although CNNs excel at extracting local features, they face limitations in modeling long-range dependencies and processing large-scale datasets. On the other hand, while Transformer models excel at capturing global dependencies, their computational complexity grows quadratically with video length and resolution, posing considerable challenges when applied to large video datasets. Consequently, relying on either CNNs or Transformers for VQA often fails to strike an effective balance between performance and computational efficiency.

%Recently, as a novel sequence modeling architecture, Mamba \cite{paper70} has attracted widespread attention for its ability to effectively solve the computational bottleneck of traditional deep learning models when dealing with long sequences. Specifically, Mamba is essentially a State Space Model (SSM) \cite{paper71,paper72,paper73,paper74,paper75,paper76} that models long-range dependencies in time-series data through a set of state transfer equations.
%Notably, the computational complexity of SSM grows linearly with the length of the input sequence. In addition to its advantages in temporal modeling, Mamba has also demonstrated outstanding performance in visual tasks \cite{paper82,paper83,paper84,paper85,paper86,paper87}, suggesting that it possesses not only strong temporal modeling capabilities but also excellent spatio-temporal awareness.
%In the context of VQA, the advantages of Mamba are particularly prominent. Videos typically contain a substantial amount of redundant information, and traditional VQA methods may suffer from reduced efficiency and accuracy due to excessive computational burden. However, the linear time complexity of the Mamba-based model allows VQA systems to efficiently process large-scale video data while accurately capturing spatio-temporal relationships and semantic features. This is especially beneficial when dealing with long-duration and high-resolution videos, where Mamba significantly enhances processing efficiency while maintaining high-quality evaluation accuracy. Therefore, Mamba-based VQA methods provide a practical and effective solution for efficient and precise video quality assessment.

Mamba \cite{paper70}, a novel sequence modeling architecture, has gained attention for addressing computational bottlenecks in processing long sequences. As a State Space Model (SSM) \cite{paper71,paper72,paper73,paper74,paper75,paper76}, Mamba models long-range dependencies with state transfer equations and linear complexity relative to input length. Beyond temporal modeling, Mamba also excels in spatio-temporal tasks \cite{paper82,paper83,paper84,paper85,paper86,paper87}, making it particularly advantageous for VQA. Traditional VQA models often struggle with redundant video data and high computational demands, but Mamba’s efficiency allows it to handle large-scale video data accurately and with reduced processing time, especially for long and high-resolution videos. Thus, Mamba-based VQA offers a practical solution for efficient and precise video quality assessment.


Moreover, the computational complexity and accuracy of VQA models are influenced not only by the model architecture but also by the sampling strategy employed. 
Traditional sampling methods like cropping \cite{paper77,paper78} and resizing \cite{paper79} reduce computational load but often distort video quality. To better retain quality information, Wu et al. \cite{paper29} introduced Grid Mini-patch Sampling (GMS), which samples small patches across uniform grids to preserve quality and temporal features. However, the fragmentation from grid sampling limits semantic information capture, which is essential for VQA accuracy \cite{paper21,paper15,paper22,paper23,paper80,paper81}. Thus, an effective sampling strategy should maintain both video quality and semantic information.
%
%
%Traditional sampling techniques, such as cropping \cite{paper77,paper78} and resizing \cite{paper79}, while effective in reducing computational overhead, often introduce significant distortions to the video quality, which in turn can negatively impact model performance.
%To effectively preserve the quality information of the original video after sampling, Wu et al. \cite{paper29} proposed Grid Mini-patch Sampling (GMS), which samples small patches from uniformly divided grids within the video frames to retain certain quality and temporal features. While this method effectively preserves video quality information, the fragmentation introduced by grid sampling makes it difficult to capture the semantic information of the video effectively. 
%However, some studies \cite{paper21,paper15,paper22,paper23,paper80,paper81} have shown that semantic information plays a crucial role in VQA, as it provides richer contextual insights, particularly when assessing video quality. Therefore, to more accurately evaluate video quality, the sampling strategy should not only comprehensively reflect the quality characteristics of the video but also retain as much of the semantic information as possible.
%
%VQA model performance depends on both architecture and sampling strategy. Traditional sampling methods like cropping \cite{paper77,paper78} and resizing \cite{paper79} reduce computational load but often distort video quality. To better retain quality information, Wu et al. \cite{paper29} introduced Grid Mini-patch Sampling (GMS), which samples small patches across uniform grids to preserve quality and temporal features. However, the fragmentation from grid sampling limits semantic information capture, which is essential for VQA accuracy \cite{paper21,paper15,paper22,paper23,paper80,paper81}. Thus, an effective sampling strategy should maintain both video quality and semantic information.

\begin{figure}[t]
	\centering
	\setlength{\abovecaptionskip}{0.1cm}
	\includegraphics[scale=0.07]{1.5.png}
	\caption{Comparison of semantic information retained by USDS with different samples (resize, Fragments \cite{paper29}).}
	\label{fig1.5}
	\vspace{-0.4cm}
\end{figure}


Based on the above analysis, we propose \textbf{U}nified \textbf{S}emantic and \textbf{D}istortion \textbf{S}ampling \textbf{(USDS)}, which not only effectively samples video distortions but also preserves the semantic information of the video.
As shown in \cref{fig1.5}, we use CLIP \cite{paper24}, with its strong zero-shot prediction capabilities, to verify that USDS effectively preserves semantic information.
Specifically, USDS first obtains a downsampled version to capture the semantic information of the video, then performs grid sampling to capture the distortion information. These two sampled maps are then combined at a specified ratio through masking.  Additionally, we introduce MVQA, a VQA model fully based on state space models, and experiments demonstrate that our model achieves a balance between performance and efficiency. As shown in \cref{fig1}, Compared to the current most efficient model, FastVQA, our MVQA-tiny achieves comparable performance while offering faster computation speed and lower memory usage.

Our contributions can be summarized as follows:
\begin{itemize}
	%	\item To the best of our knowledge, this work is the first attempt to apply state-space models in the VQA domain.
	%	\item We propose a novel sampling method, USDS, which introduces semantic information through masking fusion applied to distortion sampling. This approach overcomes the limitations of previous methods that could not account for both video distortion and semantic simultaneously.
	%%	A novel sampling method, USDS, is proposed, which introduces semantic information through masking fusion on top of distortion sampling. This approach addresses the limitation of previous sampling methods, which failed to simultaneously account for both video distortion and semantic content.
	%	\item We propose the first Mamba-based VQA model, MVQA, which effectively balances computational efficiency and modeling capacity.
	%	\item Extensive experiments show that MVQA surpasses state-of-the-art methods while ensuring efficient computation and smaller memory usage.
	\item To the best of our knowledge, this is the first work to successfully apply state-space models in the VQA domain, which effectively balances computational efficiency and performance. 
	\item We propose a novel sampling method, USDS, which unifies semantic and distortion patch sampling through masked fusion. This approach addresses the limitation of previous sampling methods, which failed to simultaneously account for both semantic content and distortions.
	\item We conduct extensive experiments to demonstrate that MVQA outperforms both transformer-based and CNN-based methods, while ensuring efficient computation and smaller memory usage.
	
\end{itemize}



%
%Traditional VQA methods mainly rely on hand-designed features, and while these methods have low computational complexity and high efficiency, they tend to have limited performance in dealing with high-resolution videos with rich details and diverse contents because they cannot effectively capture complex and high-dimensional features in videos.Comparatively, deep learning-based VQA methods, especially Convolutional Neural Networks (CNNs) and Transformer, show significant advantages in processing complex video tasks.Nonetheless, deep learning-based methods usually require high computational overheads, including huge memory consumption and long computational processes, which is particularly prominent when dealing with large-scale, high-resolution video data.
%Specifically, while CNNs can effectively extract local features, they have limitations in modeling long-range dependencies and handling large-scale datasets; while Transformer models, while they have advantages in capturing global dependencies, their computational complexity grows quadratically with the increase of video length and resolution, leading to greater challenges when applied on large-scale video datasets. Therefore, relying solely on CNN or Transformer for VQA often fails to guarantee performance while effectively controlling computational complexity.


%With the widespread use of high-definition portable devices and advances in video compression and network technologies, users can easily capture and upload long-duration, high-resolution (2K, 4K) videos. However, issues such as blur, noise, and color degradation often arise during acquisition, transmission, and processing, significantly affecting video quality. The increasing length and size of videos pose significant challenges for quality assessment algorithms. Therefore, developing efficient methods to rapidly evaluate large volumes of video data and ensure a high-quality viewing experience has become an urgent challenge.






==> ICCV2025-Author-Kit-Feb/2_related.tex <==
\section{Related Work}
\label{sec:formatting}

\subsection{VQA Methods}

Current VQA methods are mainly divided into two categories: traditional and deep learning-based methods.

Traditional VQA methods \cite{paper33,paper11,paper10,paper8,paper7} tend to be knowledge-driven, which evaluate the video quality by extracting hand-crafted features from spatial and temporal domains.
Earlier VQA \cite{paper11,paper33}  often extracts spatial features of video frames with the help of IQA algorithms \cite{paper30,paper31,paper32,paper38,paper39,paper40} and then predicts the video quality by feature aggregation.
In addition, VQA through natural video statistics (NVS) is also a classic class of VQA methods \cite{paper11,paper10,paper8,paper7}.
However, the performance is limited because hand-crafted features often fail to extract complex features from videos.

%Deep learning-based VQA methods tend to be data driven. In recent years, a large number of subjective experiments have provided several large-scale and high-quality VQA datasets \cite{paper1,paper2,paper3,paper16,paper5,paper6}, which have led to excellent performance of deep learning-based VQA methods \cite{paper41,paper15,paper42,paper16,paper17,paper18,paper29,paper23,paper43,paper19,paper45,paper46,paper20,paper68,paper69}.
%Current deep VQA methods are categorized into two main architectures, convolutional neural networks (CNN) \cite{paper47,paper48,paper49,paper50,paper51,paper52,paper55,paper56} and Transformer \cite{paper44,paper53,paper54}.
%For example, GST-VQA \cite{paper41} uses VGG \cite{paper47} to extract spatial features of frames and uses GRU \cite{paper58} for temporal modeling.
%Similar to GST-VQA, VSFA \cite{paper15} utilizes a pre-trained ResNet-50 \cite{paper48} to extract spatial features from video frames and employs a GRU model to obtain frame-level quality scores.
%Additionally, several studies \cite{paper16,paper18,paper22,paper43,paper62,paper42} have explored the use of 3D-CNNs to obtain spatiotemporal features for more comprehensive video analysis.
%Due to the success of ViTs \cite{paper44}, VQA methods \cite{paper23,paper29,paper19} based on the Transformer architecture have gradually become a current research focus.
%For example, FAST-VQA \cite{paper29} and FasterVQA \cite{paper19} obtain fragments by spatial-temporal grid mini-cube sampling (St-GMS) and then feed the fragments into a modified Video Swin Transformer \cite{paper53}.
%Although the previous methods \cite{paper29,paper19} achieved very great success in VQA, but their fragment  sampling strategy resulted in almost losing the semantic information of the video.
%Recent research \cite{paper63,paper64,paper45,paper80} often addresses this issue by adding a branch dedicated to extracting semantic information.
%For example, Dover \cite{paper64} introduces an aesthetic branch. Similar to dover, Zoom-VQA \cite{paper45} introduces an additional CNN branch.
%CLiF-VQA \cite{paper80} adds a branch to capture human feelings responses, using CLIP to extract semantic features aligned with linguistic prompts.

Deep learning-based VQA methods are primarily data-driven. Recently, numerous subjective experiments have produced large, high-quality VQA datasets \cite{paper1,paper2,paper3,paper16,paper5,paper6}, advancing deep VQA performance \cite{paper41,paper15,paper42,paper16,paper17,paper18,paper29,paper23,paper43,paper19,paper45,paper46,paper20,paper68,paper69}. Current VQA methods use either CNNs \cite{paper47,paper48,paper49,paper50,paper51,paper52,paper55,paper56} or Transformer architectures \cite{paper44,paper53,paper54}. For example, GST-VQA \cite{paper41} and VSFA \cite{paper15} employ CNNs like VGG \cite{paper47} and ResNet-50 \cite{paper48} with GRU for temporal modeling, while other studies \cite{paper16,paper18,paper22,paper43,paper62,paper42} use 3D-CNNs for spatiotemporal features. With the success of ViTs \cite{paper44}, Transformer-based VQA \cite{paper23,paper29,paper19} has gained prominence. Methods like FAST-VQA \cite{paper29} and FasterVQA \cite{paper19} sample spatial-temporal grids and utilize modified Video Swin Transformers \cite{paper53}. However, these fragment sampling strategies often neglect semantic content. Recent studies \cite{paper63,paper64,paper45,paper80} address this by adding branches for semantic extraction, such as the aesthetic branch in DOVER \cite{paper64}, a CNN branch in Zoom-VQA \cite{paper45}, and a CLIP-based branch in CLiF-VQA \cite{paper80} for aligning semantic features with linguistic prompts.

%
%\subsection{Deep Learning-based VQA Methods}
%Deep learning-based VQA methods tend to be data driven. In recent years, a large number of subjective experiments have provided several large-scale and high-quality VQA datasets \cite{paper1,paper2,paper3,paper16,paper5,paper6}, which have led to excellent performance of deep learning-based VQA methods \cite{paper41,paper15,paper42,paper16,paper17,paper18,paper29,paper23,paper43,paper19,paper45,paper46,paper20,paper68,paper69}.
%Current deep VQA methods are categorized into two main architectures, convolutional neural networks (CNN) \cite{paper47,paper48,paper49,paper50,paper51,paper52,paper55,paper56} and Transformer \cite{paper44,paper53,paper54}.
%For example, GST-VQA \cite{paper41} uses VGG \cite{paper47} to extract spatial features of frames and uses GRU \cite{paper58} for temporal modeling.
%Similar to GST-VQA, VSFA \cite{paper15} utilizes a pre-trained ResNet-50 \cite{paper48} to extract spatial features from video frames and employs a GRU model to obtain frame-level quality scores. These scores are then aggregated using a temporal pooling model.
%Using 2D-CNNs to extract spatial features followed by temporal modeling does not sufficiently capture the motion information between video frames. Consequently, some studies \cite{paper16,paper18,paper22,paper43,paper62,paper42} have explored the use of 3D-CNNs to obtain spatiotemporal features for more comprehensive video analysis.
%For example, V-MEON \cite{paper42} proposes a multitasking architecture based entirely on 3D-CNN, which not only predicts the quality of the video, but also the type of codec.
%Other studies \cite{paper16,paper22,paper43,paper18} predict video quality scores by using 2D-CNN to extract spatial features within frames and 3D-CNNs to capture inter-frame motion features, and then aggregating these two features.
%Due to the success of ViTs \cite{paper44}, VQA methods \cite{paper23,paper29,paper19} based on the Transformer architecture have gradually become a current research focus.
%DisCoVQA \cite{paper23} uses Video Swin Transformer \cite{paper53} to extract multi-level spatio-temporal features and improves the learning efficiency of the model by temporal sampling of the features.
%Similarly, FAST-VQA \cite{paper29} and FasterVQA \cite{paper19} obtain fragments by spatial-temporal grid mini-cube sampling (St-GMS) and then feed the fragments into a modified Video Swin Transformer \cite{paper53}.
%Although the previous methods \cite{paper29,paper19} achieved very great success in VQA, but their fragment  sampling strategy resulted in almost losing the semantic information of the video. 
%However the semantic information of the video is very important in VQA task \cite{paper21,paper15,paper22,paper23,paper80,paper81}, thus some works \cite{paper63,paper64,paper80,paper45} try to introduce semantic information to improve these methods.
%Specifically, MaxVQA \cite{paper63} captures a variety of quality factors that can be observed by humans through a modified vision-language foundation model CLIP and can jointly evaluate multiple specific quality factors and overall perceptual quality scores.
%Dover \cite{paper64} further introduces an aesthetic branch to extract the semantic information of the video based on the original technical branch.
%Similar to dover, Zoom-VQA \cite{paper45} introduces an additional CNN branch.
%CLiF-VQA \cite{paper80} introduces a branch designed to capture human emotional responses from videos, utilizing the CLIP model to extract semantic features closely aligned with human feelings guided by linguistic prompts.


\subsection{State Space Models}
In recent years, state space models (SSMs) \cite{paper71,paper74,paper75} have emerged as one of the primary contenders to CNN and Transformer architectures within the field of deep learning.
Originally derived from classical control theory \cite{paper88}, SSMs have attracted a great deal of interest from researchers due to their great potential for remote dependency modeling and the linear growth of model complexity with respect to sequence length.
Structured state space models (S4) \cite{paper71} introduce a diagonal structure to SSMs and combine it with the diagonal plus low rank method, which improves the computational efficiency of SSMs.
Building on this, a series of studies have enhanced the S4 model to further improve its effectiveness and efficiency.
For example, S5 \cite{paper75} further introduces MIMO SSM and efficient parallel scanning in S4.
\cite{paper76} presents a new SSM layer, H3, that greatly improves the effectiveness of SSM for language modeling.
GSS \cite{paper72} builds a gated state space layer by introducing gating mechanisms in S4 to enhance its modeling capabilities.
Recently, Mamba \cite{paper70} has refined the S4 model, a data-dependent State Space Model (SSM) that incorporates efficient hardware design and a selectivity mechanism. This enhancement allows it to outperform Transformer-based models in natural language processing tasks, while also scaling linearly in complexity with input length.
Inspired by the success of mamba, a large amount of work has successfully applied mamba to a variety of vision tasks, including image understanding \cite{paper84,paper89,paper90}, video understanding \cite{paper82,paper83,paper91}, segmentation \cite{paper92,paper93}, restoration \cite{paper94,paper95,paper96}, and others \cite{paper97,paper98,paper99,paper100,paper101}. All the studies show that mamba has better performance and higher computational efficiency than CNN and Transformer models in vision tasks.






==> ICCV2025-Author-Kit-Feb/3_approach.tex <==
\section{Approach}

\begin{figure*}[t]
	\centering
	\setlength{\abovecaptionskip}{0.1cm}
	\begin{subfigure}{0.30\linewidth}
		\centering
		\includegraphics[scale=0.113]{2.1.png}
		\caption{Unified Semantic and Distortion Sampling.}
		\label{fig3-a}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.67\linewidth}
		\centering
		\includegraphics[scale=0.113]{2.2.png}
		\caption{The network architecture of our MVQA.}
		\label{fig3-b}
	\end{subfigure}
	\caption{The framework of our proposed method. (a) The USDS consists of three distinct but interrelated stages: distortion details extraction, semantic information retention, and fusion of all resolutions. (b) MVQA transforms the input image blocks into one-dimensional vectors by 3D embedding and adds spatial location embedding and temporal location embedding to them, then extracts the features of the video using a bidirectional vision mamba encoder \cite{paper84}, and finally predicts the quality scores of the video by regressing the header. }
	\label{fig3}
	\vspace{-0.4cm}
\end{figure*}

\subsection{Preliminaries}
\textbf{State Space Models. } 
%State Space Models (SSMs) are gradually becoming one of the main model architectures in deep learning.
State Space Models (SSMs) are inspired by the continuous linear time-invariant (LTI) systems, which maps an input sequence $ x(t)\in \mathbb{R}^{L} $ to a latent spatial representation $ h(t)\in \mathbb{R}^{N} $ and then predicts an output sequence  $ y(t)\in \mathbb{R}^{L} $ based on that representation.
Formally, SSMs can be formulated as a linear ordinary differential equation (ODE) as follows:
\begin{align}
	h^{'}(t) &= Ah(t)+Bx(t)\\
	y(t) &= Ch(t)+Dx(t)
	\label{Eq.1}
\end{align}
where N is the dimension of the hidden state, $ h(t)\in \mathbb{R}^{N} $ is a hidden state, $ A \in \mathbb{R}^{N\times N} $ is the evolution parameter, $ B \in \mathbb{R}^{N} $ and $ C \in \mathbb{R}^{N} $ are the projection parameters,  $ D \in \mathbb{R}^{1} $ represents the skip connection.


\noindent
\textbf{Discretization.}
To process discrete inputs, the Zero-Order Holding (ZOH) rule is often utilized, which uses the sample timescale parameters $ \bigtriangleup $ to convert the continuous parameters $ A $ and $ B $ in the ODE to discrete parameters $ \overline{A} $ and $ \overline{B} $:
%
%In order to facilitate the processing of discrete data such as text, images, etc., a continuous system of SSMs needs to be subjected to discretization operations. 
%Specifically, the discretization process follows the zero-order hold (ZOH) rule, which uses the sample timescale parameters $ \bigtriangleup $ to convert the continuous parameters $ A $ and $ B $ in the ODE to discrete parameters $ \overline{A} $ and $ \overline{B} $.  
%The formulaic representation of the discretization is as follows:
%The discretization formula is as follows:
\begin{align}
	\overline{A} &= exp(\bigtriangleup A) \\
	\overline{B} &= (\bigtriangleup A) ^{-1} (exp(A)-I)\cdot \bigtriangleup B
\end{align}
where $ \overline{A}\in \mathbb{R}^{N\times N} $, $ \overline{B}\in \mathbb{R}^{N} $.
This results in the following discretized OED formula:
\begin{align}
	h_{k} &= \overline{A}h_{k-1} + \overline{B}x_{k} \\
	y_{k} &= Ch_{k} + Dx_{k}  
\end{align}

Then in order to increase the computational speed, global convolutional operations with the advantage of parallel computing are utilized to accelerate the above computational process:
\begin{align}
	\label{Eq2}
	\overline{K} &\triangleq (C{\overline{B}} ,C\overline{AB},\cdot \cdot \cdot ,C\overline{A}^{L-1}\overline{B}) \\
	y &= x \circledast \overline{K} 
\end{align}
where $ L $ is the length of the input sequence, $\circledast$ denotes convolution operation, and $\overline{K} \in \mathbb{R}^{L} $ is a structured convolutional kernel.
%This allows the global convolution to be utilized to process the entire input sequence at the same time, greatly improving computational efficiency.

%\noindent
%\textbf{Selective State Space Models.} 
%Since traditional SSMs employ constant transition parameters ($\overline{A}$ and $\overline{B}$), this limits the ability of the model to be used in sequence modeling.
%To address this limitation, Mamba \cite{paper70} based on the selective state space model (S6) establishes an input dependency mechanism for the parameters $\overline{B}$, $\overline{C}$, and $\bigtriangleup $, which allows these parameters to be dynamically updated based on the inputs, thus improving the performance of the model based on SSMs.
%With the introduction of the input dependency mechanism, the global convolution operation in Eq. \eqref{Eq2} is represented as:
%
%\begin{equation}
%	\overline{K} = \big( C_{L}\overline{B}_{L}, C_{L}\overline{A}_{L-1}\overline{B}_{L-1},\cdot \cdot \cdot ,C_{L}\prod_{i=1}^{L-1}\overline{A} _{i} \overline{B}_{1}      \big)
%\end{equation}




\subsection{Overall Architecture}
The architecture proposed in this paper consists of two main components: the unified semantic and distortion sampling (USDS) and the MVQA model design (\cref{fig3}). Previous studies \cite{paper29,paper19,paper102,paper23,paper103} have shown that effective sampling not only reduces model complexity but also improves performance. However, prior methods often lose critical semantic information due to fragmentation in sampled segments, affecting quality prediction. To solve this, we introduce USDS (\cref{fig3-a}), which samples video at its original resolution for distortion and downsamples for semantic information. These are fused through mask fusion to form the final sampled video. The MVQA model then uses 3D embedding on USDS results (\cref{fig3-b}), adding a regression token for quality prediction. Spatial and temporal embeddings are successively added, and the vision Mamba encoder extracts features for final quality scoring based on the regression token.

%The architecture of the methods proposed in this paper consists of two main parts, i.e., the unified semantic and distortion sampling (USDS) and the design of the MVQA model, as shown in Fig. \ref{fig3}.
%
%Several VQA research \cite{paper29,paper19,paper102,paper23,paper103} has demonstrated that a good sampling strategy not only reduces the computational complexity of the model, but also leads to better performance.
%Although these methods have achieved satisfactory results, the characteristics of their sampling strategies have led to severe fragmentation between the sampled segments, almost losing the semantic information in the video that has an important impact on quality prediction.
%To address this problem, we propose a unified semantic and distortion sampling approach, as shown in Fig. \ref{fig3-a}, which involves sampling the video at its original resolution to capture distortion information and downsampling to extract semantic information. These two sampling results are then fused through mask fusion to produce the final sampled video.
%Moreover, our MVQA model takes the sampling results of USDS as inputs and maps the inputs by 3D embedding, as shown in Fig. \ref{fig3-b}. An additional regression token is then added to the sequence to be used for final video quality prediction. In order for the model to better model the intra- and inter-frame relationships of the video, spatial location embedding and temporal embedding are successively added to the input sequences, and then the features with temporal and spatial embedding are fed into the vision mamba encoder for feature extraction. Finally, the output corresponding to the regression token is regressed and analyzed to obtain the predicted quality score of the video.


\subsection{Unified Semantic and Distortion Sampling}
\begin{figure*}[t]
	\vspace{-0.4cm}
	\centering
	\setlength{\abovecaptionskip}{0.1cm}
	\includegraphics[scale=0.15]{3.1.png}
	\caption{Comparison of USDS with crop, resize, MRET \cite{paper102}, Fragments \cite{paper29} sampling.}
	\label{fig2}
	\vspace{-0.4cm}
\end{figure*}

Considering the significant computational burden associated with model learning, we propose an approach that integrates high-resolution visual details with low-resolution semantic information to enhance the representation of video frames, which is called \textbf{U}nified \textbf{S}emantic and \textbf{D}istortion \textbf{S}ampling \textbf{(USDS)}, as shown in \cref{fig3-a}.
And the detailed USDS process is shown in \cref{alg:spatial_fragments_gms}.
%And the USDS process is visualized in \cref{fig3-a}. 

%The USDS consists of three distinct but interrelated stages: distortion details extraction, semantic information retention, and fusion of resolutions, each designed to enhance the representation of spatial features in video data.

%Given the substantial computational overhead of fragment-based sampling in model training, as noted in FastVQA~\cite{fastvqa}, we draw inspiration from MRET~\cite{MRET}---a multi-scale video representation method used in Video Quality Assessment (VQA)---to propose a novel approach: \textbf{U}nified \textbf{S}emantic and \textbf{D}istortion \textbf{S}ampling (USDS). This method integrates high-resolution visual details with low-resolution semantic information to create a comprehensive representation of video frames. USDS operates in two interconnected stages---distortion detail extraction and semantic information fusion---each designed to enhance the spatial feature representation in video data.
\noindent
\textbf{Distortion Details and Semantic Information Extraction.}
In the first stage, input video frames $ V \in \mathbb{R}^{C \times T \times H \times W} $ are partitioned into high-resolution spatial fragments. The target resolution, denoted as $ S_h = fragments_h \times fsize_h $ and $ S_w = fragments_w \times fsize_w $ (e.g., $ 14 \times 16 = 224 $ for both), is achieved by dividing the frame into a grid of $ fragments_h \times fragments_w $ patches, each of size $ fsize_h \times fsize_w $. These fragments are sampled with random spatial offsets within each grid cell, preserving local details such as textures and edges crucial for high-fidelity reconstruction. The grid starting points are determined by evenly dividing the height and width, adjusted to avoid exceeding the frame boundaries.

For semantic information retention, each frame is downsampled to a lower resolution, typically $ S_h / 2 \times S_w / 2 $ (e.g., $ 112 \times 112 $ when $ S_h = S_w = 224 $), using bilinear interpolation:
\begin{equation}
	V_{low}[:, t, :, :] = Resize(V[:, t, :, :], (S_h / 2, S_w / 2))
\end{equation}
This process captures global contextual features, such as object boundaries and scene structure, essential for understanding the broader video context.

\noindent
\textbf{Fusion of Resolutions.}
In the second stage, the high-resolution fragments and low-resolution semantic content are fused within a multi-resolution framework. Each frame is divided into blocks of size $ 2 \cdot fsize_h \times 2 \cdot fsize_w $ (e.g., $ 32 \times 32 $ when $ fsize_h = fsize_w = 16 $), forming a grid of $ fragments_h / 2 \times fragments_w / 2 $ blocks. The high-resolution fragments are arranged to fill an intermediate frame $ \tilde{V}[:, t, :, :] $ according to their grid positions.

The low-resolution content $ V_{low} $ is expanded into a frame $ E[:, t, :, :] \in \mathbb{R}^{C \times S_h \times S_w} $ by placing each $ fsize_h \times fsize_w $ patch into the bottom-right quadrant of the corresponding $ 2 \cdot fsize_h \times 2 \cdot fsize_w $ block:
\begin{equation}
	E[:, t, R_{k,l}] = V_{low}[:, t, k' : k' + fsize_h, l' : l' + fsize_w]
\end{equation}
where $k'=0, 1, \dots, fragments_h / 2 - 1 $, and $l'=0, 1, \dots, fragments_w / 2 - 1 $, and \( R_{k,l} \) is the bottom-right $ fsize_h \times fsize_w $ region of the block with top-left corner at $ (k' \cdot 2 \cdot fsize_h, l' \cdot 2 \cdot fsize_w) $.

\begin{algorithm}[t]
	\caption{Unified Semantic and Distortion Sampling}
	\label{alg:spatial_fragments_gms}
	\begin{algorithmic}[1]
		\REQUIRE Video tensor $V \in \mathbb{R}^{C \times T \times H \times W}$, fragments $(f_h, f_w)$, size $(s_h, s_w)$, alignment $a$
		\STATE Compute $H' = f_h s_h$, $W' = f_w s_w$
		\STATE $\tilde{V}= \text{Fragments}(V, f_h, f_w, s_h, s_w, a)$
		\STATE Create mask $M \in \{0,1\}^{1 \times 1 \times H' \times W'}$:
		\[
		M_{x,y} = 
		\begin{cases} 
			1, & (x \bmod 2s_h) \ge s_h \wedge (y \bmod 2s_w) \ge s_w \\
			0, & \text{otherwise}
		\end{cases}
		\]
		\FOR{each frame $t \in [0,T)$}
		\STATE Initialize canvas: $E \leftarrow \mathbf{0}^{C \times H' \times W'}$
		\STATE $V_\text{low} \leftarrow \text{Resize}(V[:,t], \frac{H'}{2} \times \frac{W'}{2})$
		\FOR{each $(i,j)$ in $\left(\frac{H'}{2s_h}\right) \times \left(\frac{W'}{2s_w}\right)$ grid}
		\STATE Copy $E[:, 2i s_h + s_h:2(i+1) s_h, 2j s_w + s_w:2(j+1) s_w] \leftarrow V_{\text{low}}[:, i s_h:(i+1) s_h, j s_w:(j+1) s_w]$
		\ENDFOR
		\STATE $\hat{V}[:,t] \leftarrow E \odot M + \tilde{V}[:,t] \odot (1-M)$
		\ENDFOR
		\RETURN $\hat{V}$
	\end{algorithmic}
	
\end{algorithm}

A binary mask $ M \in \mathbb{R}^{1 \times 1 \times S_h \times S_w} $ is defined to select the bottom-right $ fsize_h \times fsize_w $ region of each block.
%\begin{itemize}
%	\item \( M[0, 0, y, x] = 1 \) if \( (k \cdot 2 \cdot fsize_h + fsize_h \leq y < (k+1) \cdot 2 \cdot fsize_h) \land (l \cdot 2 \cdot fsize_w + fsize_w \leq x < (l+1) \cdot 2 \cdot fsize_w) \) for \( k = 0, 1, \ldots, fragments_h / 2 - 1 \) and \( l = 0, 1, \ldots, fragments_w / 2 - 1 \),
%	\item \( M[0, 0, y, x] = 0 \) otherwise.
%\end{itemize}
The fusion combines $ E \) and \( \tilde{V} $ for each frame $ t $:
\begin{equation}
	\hat{V}[:, t, :, :] = E[:, t, :, :] \cdot M + \tilde{V}[:, t, :, :] \cdot (1 - M)
\end{equation}
where $ \hat{V} \in \mathbb{R}^{C \times T \times S_h \times S_w} $ is the final output, blending high-resolution details in three quadrants with low-resolution semantic information in the bottom-right quadrant of each block.

The fused fragments are reassembled into complete video frames, producing the output \( \hat{V} \). \cref{fig2} illustrates a comparison between USDS and other sampling methods. By preserving fine-grained textures in high-resolution patches while integrating global semantic context from low-resolution data, USDS achieves a balanced representation that enhances both visual quality and semantic consistency. 







%\subsection{Unified Semantic and Distortion Sampling} 
%
%
%Considering the significant computational burden associated with model learning in fragment sampling, we draw inspiration from MRET \cite{paper102}, a multi-scale video representation method employed in VQA, and propose an approach that integrates high-resolution visual details with low-resolution semantic information to enhance the representation of video frames, which is called \textbf{U}nified \textbf{S}emantic and \textbf{D}istortion \textbf{S}ampling (USDS), as shown in \cref{fig3-a}. The USDS consists of three distinct but interrelated stages: distortion details extraction, semantic information retention, and fusion of resolutions, each designed to enhance the representation of spatial features in video data.
%
%\noindent
%\textbf{Distortion Details Extraction. } 
%Following the strategy outlined in \cite{paper29}, we divide the input video frames into uniform grids and then sample a small fragment from each grid.
%This fragmentation ensures that each spatial block contains a sufficient amount of local information, allowing for the preservation of fine details and textures crucial for high-fidelity video reconstruction.
%
%
%
%\noindent
%\textbf{Semantic Information Retention. }
%To preserve the semantic information of the video, we downsample the video frames to a lower resolution using bilinear interpolation.
%This reduction captures global semantic information, such as object boundaries and scene structure, which aids in understanding the larger context of the video. After resizing, the low-resolution frames may be upsampled to match the dimensions of the high-resolution frames, ensuring spatial alignment between the two resolutions. The process of inserting low-resolution content into the bottom-right corner of a high-resolution frame can be described as follows. Let $V_{low}$  represent the low-resolution frame of size $H_{low}\times W_{low}$ , and $V_{target}$ denote the target high-resolution frame of size $H_{target}\times W_{target}$. Using a binary mask $A[i,j]$, the low-resolution content is inserted into the bottom-right corner of the high-resolution frame, and all other regions are filled with zeros. The process is mathematically expressed as:
%\begin{equation}
%	V_{target}[i,j] = \left\{\begin{matrix}
%		V_{low}[i,j],  &if A[i,j] = 1
%		\\
%		0, &if A[i,j]=0
%	\end{matrix}\right.
%\end{equation}
%where $A[i,j]$ is the binary mask that indicates which parts of the high-resolution frame will be filled with low-resolution content, while the remaining parts are filled with zeros.
%
%\noindent
%\textbf{Fusion of Resolutions.} Each video frame is partitioned into blocks of fixed spatial size. The bottom-right region of each block, which corresponds to a specific fraction of the block's total area, is filled with the corresponding low-resolution information derived from the resized version of the original frame. A binary mask is employed to select the regions where the low-resolution content is inserted. The fusion process can be formally expressed as follows:
%\begin{equation}
%	F_{i, j}=\left(1-\mathcal{M}_{i, j}\right) \odot p_{i, j}+V_{low}[i: i+\mathrm{ps}, j: j+\mathrm{ps}]
%\end{equation}
%%\[
%%F_{i,j} = (1 - \mathcal{M}_{i,j}) \odot p_{i,j} +  V_{\text{low}}[i:i+\text{ps}, j:j+\text{ps}]
%%\]
%where $ \mathcal{M}_{i,j} $ represents the binary mask that specifies the position of the low-resolution content, \( p_{i,j} \) corresponds to the high-resolution fragment, ps means the patch\_size, $ V_{\text{low}} $ refers to the low-resolution video, and $ F_{i,j} $ denotes the resulting fused fragment. This fusion technique integrates high-resolution details from the original video with semantic information captured from the low-resolution representation, enhancing both local fine-grained textures and the broader global context of the scene.
%
%Finally, the fused fragments are reassembled to reconstruct the complete video frames, producing the output video. \cref{fig2} shows the shows the comparison between our sampling method and others. This multi-resolution fusion strategy leverages the complementary strengths of both high- and low-resolution information, thereby enhancing the visual quality and semantic consistency of the video content. By maintaining high-resolution detail in local regions while integrating low-resolution semantic features in larger blocks, USDS provides a robust solution for video processing tasks requiring both fine-grained and global contextual understanding.


\subsection{MVQA Model}
\cref{fig3-b} shows the structure of the proposed MVQA.
Since the mask fusion in our sampling operation is performed in terms of sample block size, we chunk the input strictly according to the sample size in order to better preserve the quality information and semantic information of the original video carried in the sampled video.
Since chunking the input destroys the spatio-temporal information of the video, in order to better model the intra-frame and inter-frame information of the input video,  we follow \cite{paper83} to add spatial position embedding for sequences within the input frames and temporal position embedding for sequences between frames.
Specifically, each input block of samples is processed using 3D convolution, where the size of the convolution kernel is $1\times 16 \times 16$. For an input video of size $X^{I}\in \mathbb{R} ^{3\times T \times H \times W} $, features of size $X^{o}\in \mathbb{R} ^{L \times C} $ are obtained after convolution, where $ L = T \times \frac{H}{16} \times \frac{W}{16}$.
Then a regression token for final quality regression and positional embedding are added to the token sequence :
\begin{equation}
	X = [ X_{reg},X ] + p_{s} + p_{t} 
\end{equation}
where $ X_{reg} $ is a learnable token that is prepended to the start of the sequence, $ p_{s}\in \mathbb{R}^{(\frac{H}{16} \times \frac{W}{16} +1)\times C}  $ is a learnable spatial position embedding, $p_{t}\in \mathbb{R}^{t\times C}  $  is a learnable temporal position embedding.

Then, we feed the sequence of tokens $ X $ into the vision mamba encoder to pass:
\begin{equation}
	T_{l} = Vim(T_{l-1} + T_{l-1}  ) 
\end{equation}
where $Vim$ represents the vision mamba block \cite{paper84} and $l$ represents the current number of layers.

Finally, we normalize the out put regression token $ X^{0}_{L} $ and feed it to the multi-layer perceptron (MLP) head to obtain the final prediction of the video quality score $ Q $ as follows:
\begin{equation}
	f = Norm(X^{0}_{L}),
	Q = MLP(f)
\end{equation}
where $ L $ denotes the number of layers of vision mamba block.

%Vision mamba \cite{paper84} introduces a bidirectional scanning mechanism into mamba, which processes the input token sequence forward and backward at the same time, effectively enhancing the ability of mamba spatial modeling, and this mechanism shows very good results on image data tasks with spatial location information.
%However, video data not only has spatial location relationship, but also has temporal information to be modeled.
%Designing an effective scanning mechanism plays a crucial role in the performance of the model.
%Fortunately, Li et al. \cite{paper83} explored the effect of different scanning mechanisms on video tasks and found that the simplest first spatial scanning then temporal scanning mechanism was the most effective, so we continue to follow this scanning mechanism in MVQA, as shown in Fig. \ref{fig4}.

Vision Mamba \cite{paper84} introduces a bidirectional scanning mechanism that processes tokens forward and backward, enhancing Mamba's spatial modeling and yielding strong results on image tasks. However, video data requires both spatial and temporal modeling. Li et al. \cite{paper83} found that a spatial-first, temporal-next scanning approach is most effective for video tasks, so MVQA adopts this mechanism, as shown in \cref{fig4}.


\begin{figure}[t]
	\centering
	\setlength{\abovecaptionskip}{0.1cm}
	\includegraphics[scale=0.17]{2.3.png}
	\caption{Scan method.}
	\label{fig4}
	\vspace{-0.4cm}
\end{figure}

\begin{table*}[h]
	\vspace{-0.4cm}
	\setlength{\abovecaptionskip}{0.01cm} %调节表格和标题的距离
	\caption{Experimental performance of the pre-trained MVQA model on the LSVQ dataset on four test sets (LSVQ$_{test}$, LSVQ$_{1080p}$, KoNViD-1k, LIVE-VQC). 
		%		LSVQ$_{test}$ and LSVQ$_{1080p}$ are used for intra-dataset testing.
		%		While KoNViD-1k and LIVE-VQC are used for cross-dataset testing. 
		Existing best multi-branch in \textbf{\textcolor{green!50!black}{green}} and existing best single-branch in \textbf{\textcolor{blue}{blue}}.}
	\centering
	\label{table1}
	\small
	
	\setlength{\aboverulesep}{0pt}
	\setlength{\belowrulesep}{0pt}
	\renewcommand\arraystretch{0.9}
	\centering\setlength{\tabcolsep}{5.1pt}
	
	\begin{tabular}{c|c|c|cc|cc|cc|cc}
		\toprule
		\multicolumn{3}{c|}{Testing Type} & \multicolumn{4}{c|}{Intra-dataset Test Datasets} & \multicolumn{4}{c}{Cross-dataset Test Datasets} \\
		\hline
		\multicolumn{3}{c|}{Testing Datasets} & \multicolumn{2}{c|}{\textbf{LSVQ$_{test}$}} & \multicolumn{2}{c|}{\textbf{LSVQ$_{1080p}$}} & \multicolumn{2}{c|}{\textbf{KoNViD-1k}} & \multicolumn{2}{c}{\textbf{LIVE-VQC}} \\
		\hline
		Type & Methods & Source & SROCC & PLCC & SROCC & PLCC & SROCC & PLCC & SROCC & PLCC \\
		\hline
		\multirow{3}{*}{Classical} & BRISQUE \cite{paper30} &\footnotesize \itshape TIP, 2012 &  0.569 & 0.576  & 0.497  & 0.531  & 0.646  & 0.647  & 0.524  & 0.536 \\ 
		& TLVQM \cite{paper8} &\footnotesize \itshape TIP, 2019 & 0.772 & 0.774  & 0.589  & 0.616  & 0.732  & 0.724  & 0.670  & 0.691 \\ 
		& VIDEVAL \cite{paper7} &\footnotesize \itshape TIP, 2021 &  0.794 & 0.783  & 0.545  & 0.554  & 0.751  & 0.741  & 0.630  & 0.640 \\ 
		\hdashline
		\multirow{6}{*}{\shortstack{Deep \\ Multi-branch}} 
		& PVQ$_{wo/patch}$ \cite{paper16} & \footnotesize\itshape CVPR, 2021 &  0.814 & 0.816  & 0.686  & 0.708  & 0.781  & 0.781  & 0.747  & 0.776 \\ 
		& PVQ$_{w/patch}$ \cite{paper16} &\footnotesize\itshape  CVPR, 2021 &  0.827 & 0.828  & 0.711  & 0.739  & 0.791  & 0.795  & 0.770  & 0.807 \\
		& BVQA \cite{paper17} & \footnotesize\itshape TCSVT, 2022 &  0.852 & 0.854  & 0.771  & 0.782  & 0.834  & 0.837  & 0.816  & 0.824 \\
		& DOVER  \cite{paper64}& \footnotesize\itshape ICCV, 2023 &  0.881 & 0.879  & 0.782  & 0.827  & 0.871  & 0.872  & 0.812  & 0.841 \\
		& Zoom-VQA \cite{paper45} & \footnotesize\itshape CVPR,2023 & 0.886 & 0.879 & 0.799  & 0.819 & 0.877 & 0.875 & 0.814 & 0.833 \\
		%		& A$^2$INet \cite{paper104}& \footnotesize\itshape ACMMM,2024 &  0.878 & 0.878  & 0.785  & 0.818  & 0.867  & 0.864  & 0.817  & 0.815 \\
		& Q-Align \cite{paper105} & \footnotesize\itshape ICML, 2024 & 0.883  & 0.882  & 0.797  & 0.830  & 0.865  & 0.877  & NA  & NA \\
		& CLiF-VQA \cite{paper80}  & \footnotesize\itshape ACMMM,2024 &  0.886 & 0.887  & 0.790  & 0.832  & 0.877  & 0.874  & \textbf{\textcolor{green!50!black}{0.834}}  & \textbf{\textcolor{green!50!black}{0.855}} \\
		& MBVQA \cite{paper106} & \footnotesize\itshape CVPR, 2024 & \textbf{\textcolor{green!50!black}{0.895}}  & \textbf{\textcolor{green!50!black}{0.895}}  & \textbf{\textcolor{green!50!black}{0.809}}  & \textbf{\textcolor{green!50!black}{0.844}}  & \textbf{\textcolor{green!50!black}{0.878}}  & \textbf{\textcolor{green!50!black}{0.884}}  & 0.806  & 0.844 \\
		
		\hdashline
		\multirow{6}{*}{\shortstack{Deep \\ Single-branch}} & VSFA \cite{paper15}& \footnotesize\itshape ACMMM, 2019 & 0.801 & 0.796 & 0.675  & 0.704  & 0.784  & 0.794  & 0.734  & 0.772 \\ 
		& FAST-VQA-M \cite{paper29}& \footnotesize\itshape ECCV, 2022 &  0.852 & 0.854  & 0.739  & 0.773  & 0.841  & 0.832  & 0.788  & 0.810 \\
		%	FAST-VQA \cite{paper29}& ECCV, 2022 &  0.876 & 0.877  & 0.799  & 0.814  & 0.859  & 0.855  & 0.823  & 0.844 \\
		& FAST-VQA \cite{paper29}& \footnotesize\itshape ECCV, 2022 &  0.872 & \textbf{\textcolor{blue}{0.874}}  & 0.770  & 0.809  & \textbf{\textcolor{blue}{0.864}}  & 0.862  & \textbf{\textcolor{blue}{0.824}}  & \textbf{\textcolor{blue}{0.841}} \\
		
		& FasterVQA \cite{paper19}  & \footnotesize\itshape TPAMI, 2023 &  \textbf{\textcolor{blue}{0.873}} & \textbf{\textcolor{blue}{0.874}}  & \textbf{\textcolor{blue}{0.772}}  & \textbf{\textcolor{blue}{0.811}}  & 0.863  & \textbf{\textcolor{blue}{0.863}}  & 0.813  & 0.837 \\
		
		%	DOVER \cite{paper64} & ICCV, 2023 &  0.888 & 0.889  & 0.795  & 0.830  & 0.884  & 0.883  & 0.832  & 0.855 \\
		
		\cline{2-11}
		& \textbf{MVQA-tiny }  & \textbf{\itshape ours} &  \textbf{0.882} & \textbf{0.883}  & \textbf{0.781}  & \textbf{0.823}  & \textbf{0.870}  & \textbf{0.868}  & \textbf{0.828}  & \textbf{0.848} \\
		& \textbf{MVQA-middle}   & \textbf{\itshape ours} &  \textbf{\textcolor{red}{0.898}} & \textbf{\textcolor{red}{0.899}}  & \textbf{\textcolor{red}{0.812}}  & \textbf{\textcolor{red}{0.846}}  & \textbf{\textcolor{red}{0.885}}  & \textbf{\textcolor{red}{0.887}}  & \textbf{\textcolor{red}{0.852}}  & \textbf{\textcolor{red}{0.873}} \\
		\hdashline
		\multicolumn{3}{c|}{\footnotesize \itshape improvement to existing best Single-branch}  &\footnotesize \itshape \textcolor{blue}{$ 2.86\%$} &\footnotesize \itshape \textcolor{blue}{$ 2.86\%$}  &\footnotesize \itshape \textcolor{blue}{$ 5.18\%$}  &\footnotesize \itshape \textcolor{blue}{$ 4.32\%$} &\footnotesize \itshape \textcolor{blue}{$ 2.43\%$} &\footnotesize \itshape \textcolor{blue}{$ 2.78\%$} &\footnotesize \itshape \textcolor{blue}{$ 3.40\%$} &\footnotesize \itshape \textcolor{blue}{$ 3.80\%$} \\
		\hdashline
		\multicolumn{3}{c|}{\footnotesize \itshape improvement to existing best Multi-branch}  &\footnotesize \itshape \textcolor{green!50!black}{$ 0.34\% $} &\footnotesize \itshape \textcolor{green!50!black}{$ 0.45\% $}  &\footnotesize \itshape \textcolor{green!50!black}{$ 0.37\% $}  &\footnotesize \itshape \textcolor{green!50!black}{$ 0.24\% $} &\footnotesize \itshape \textcolor{green!50!black}{$ 0.80\% $} &\footnotesize \itshape \textcolor{green!50!black}{$ 0.34\% $} &\footnotesize \itshape \textcolor{green!50!black}{$ 2.16\% $} &\footnotesize \itshape \textcolor{green!50!black}{$ 2.11\% $} \\
		\bottomrule
	\end{tabular}
	\vspace{-0.4cm}
\end{table*}

\subsection{Loss Function}
Several studies have shown that both monotonicity-induced loss and linearity-induced loss play a very important role in the quality prediction task, so we combine both as our loss function.
Given the predicted quality score $ \hat{Q}=\left \{ \hat{q_{1}},\hat{q_{2}},...,\hat{q_{m}} \right \} $ and ground-truth subjective quality score $ Q=\left \{ q_{1},q_{2},...,q_{m} \right \} $.

The monotonicity-induced loss $ L_{mon} $ and the linearity-induced loss $ L_{lin} $ are defined as follows:
\begin{equation}
	L_{mon} =\frac{1}{m^{2} } \sum_{i=1}^{m} \sum_{j=1}^{m}max(0,\left | q_{i}- q_{j} \right |-f(q_{i}, q_{j})\cdot (\hat{q_{i}}-\hat{q_{j}} ) ) 
\end{equation}
where $ f(q_{i}, q_{j})=1 $ if $ q_{i}\ge q_{j} $, otherwise $ f(q_{i}, q_{j})=-1 $.

\begin{equation}
	%	L_{lin} = \left ( 1-\frac{ {\textstyle \sum_{i=1}^{m}(\hat{q}_{i}-\hat{a} )({q}_{i}-{a})} }{\sqrt{ {\textstyle \sum_{i=1}^m{(\hat{q}_{i}- \hat{a})^{2} {\textstyle \sum_{i=1}^{m}(q_{i}-a)^{2}}  }} } }  \right ) {\div} 2
	L_{lin} = ( 1-\frac{ {\textstyle \sum_{i=1}^{m}(\hat{q}_{i}-\hat{a} )({q}_{i}-{a})} }{\sqrt{ {\textstyle \sum_{i=1}^m{(\hat{q}_{i}- \hat{a})^{2} {\textstyle \sum_{i=1}^{m}(q_{i}-a)^{2}}  }} } } )/2
\end{equation}
where $ a= \frac{1}{m} {\textstyle \sum_{i=1}^{m}} q_{i} $ and $ \hat{a} = \frac{1}{m} {\textstyle \sum_{i=1}^{m}} \hat{q}_{i} $.

The total loss function $ L $ is obtained by combining the two loss functions $ L_{mon} $ and $ L_{lin} $ above:
\begin{equation}
	L=\alpha L_{mon}+\beta L_{lin}
\end{equation}
where $ \alpha $ and $ \beta $ represent the weights of monotonicity-induced loss and linearity-induced loss. 



==> ICCV2025-Author-Kit-Feb/4_experiments.tex <==
\section{Experiments}
\label{sec:5}

\subsection{Experimental Setups}

\noindent
\textbf{Datasets.} 
We test the model on four datasets including LSVQ \cite{paper16}, KoNViD-1k (1200 videos) \cite{paper1}, LIVE-VQC (585 videos) \cite{paper3}, and YouTube-UGC (1067 videos) \cite{paper6}. 
Specifically, we pre-train MVQA on LSVQ$_{train}$, a subset of  LSVQ containing 28,056 videos. 
Intra-dataset testing is performed on two subsets of LSVQ, LSVQ$_{test}$ (7400 videos) and LSVQ$_{1080p}$ (3600 videos).
We perform cross-dataset testing on KoNViD-1k and LIVE-VQC.
Further, we fine-tune the model on  KoNViD-1k, LIVE-VQC, and YouTube-UGC.
It should be noted that  YouTube-UGC contains 1500 videos, but only 1067 videos are available to us.
%We test the proposed model on four datasets including LSVQ \cite{paper16}, KoNViD-1k \cite{paper1}, LIVE-VQC \cite{paper3}, and YouTube-UGC \cite{paper6}. 
%LSVQ is the largest-scale VQA dataset to date, which obtains 38,811 real-world videos of diverse sizes, contents and distortions by sampling UGC videos from hundreds of thousands of open-source Internet. 
%We use LSVQ$_{train}$, a subset of LSVQ containing 28056 videos, to train CLiF-VQA.
%Additionally we choose LSVQ$_{test}$, LSVQ$_{1080p}$, KoNViD-1k and LIVE-VQC to test the training effect of the model. LSVQ$_{test}$ and LSVQ$_{1080p}$ are test subsets in LSVQ.
%Specifically, LSVQ$_{test}$ contains 7,400 videos of various resolutions from 240p to 720p, and LSVQ$_{1080p}$ consists of 3,600 1080p high resolution videos.
%In addition, KoNViD-1k contains 1,200 540p natural videos with a wide variety of contents and authentic distortions. 
%LIVE-VQC contains 585 videos with resolutions ranging from 240p to 1080p, which are mainly shot in natural environments with smartphones.
%Further, we fine-tune the model on  KoNViD-1k, LIVE-VQC, and YouTube-UGC.
%YouTube-UGC is composed of 1500 videos with various categories of distortion and with resolutions ranging from 360p to 4K.
%But there are only 1067 videos in YouTube-UGC available to us.

\noindent
\textbf{Evaluation Criteria.} Spearman Rank Order Correlation Coefficient (SROCC) and Pearson Linear Correlation Coefficient (PLCC) are used as evaluation Metrics. 
Specifically, SRCC is used to measure the prediction monotonicity between predicted scores and true scores by ranking the values in both series and calculating the linear correlation between the two ranked series. 
In contrast, PLCC evaluates prediction accuracy by calculating the linear correlation between a series of predicted scores and true scores.
And higher SROCC and PLCC scores indicate better performance.


\noindent
\textbf{Implementation Details.} 
We employ PyTorch framework and an NVIDIA H100 card to train the model.
We pre-train the MVQA backbone network on the Kinetics-400  \cite{paper65} dataset.
We set the initial learning rate to 0.0025, the optimizer to AdamW, and use a cosine annealing strategy to dynamically adjust the learning rate. 
The detailed information of our proposed MVQA with two different scales is shown in \cref{table0}.
For MVQA-tiny and MVQA-middle, we set the batch size to 32 and 8, and the weight decay during training to 0.1 and 0.05.

\begin{table}[t]
	\setlength{\abovecaptionskip}{0.01cm}
	\caption{Details of MVQA with different sizes.}
	\centering\setlength{\tabcolsep}{4.7pt}
	\label{table0}
	\footnotesize
	%	\small
	\setlength{\aboverulesep}{0pt}
	\setlength{\belowrulesep}{0pt}
	%	\setlength\tabcolsep{7pt}  %列间距
	
	\begin{tabular}{l|c|c|c|c|c}
		\toprule
		Models & Input Size& Depth & Dim & Param & Flops   \\
		\hline
		MVQA-tiny & $32\times224 \times 224$ & 24 & 192 & 7M & 34G    \\
		MVQA-middle & $32\times224 \times224$ & 32 & 576 & 74M & 403G   \\
		\bottomrule
	\end{tabular}
	\vspace{-0.4cm}
\end{table}

\begin{table*}[t]
	\vspace{-0.4cm}
	\setlength{\abovecaptionskip}{0.01cm} %调节表格和标题的距离
	\caption{The finetune results on LIVE-VQC, KoNViD and YouTube-UGC.
		Existing best multi-branch in \textbf{\textcolor{green!50!black}{green}} and existing best single-branch in \textbf{\textcolor{blue}{blue}}.
	}
	\label{table2}
	%\footnotesize
	\small
	\setlength{\aboverulesep}{0pt}
	\setlength{\belowrulesep}{0pt}
	\renewcommand\arraystretch{0.9}
	\centering\setlength{\tabcolsep}{4pt}
	
	\begin{tabular}{c|c|c|cc|cc|cc|cc}
		\toprule
		\multicolumn{3}{c|}{Finetune Datasets} & \multicolumn{2}{c|}{\textbf{LIVE-VQC}} & \multicolumn{2}{c|}{\textbf{KoNViD-1k}} & \multicolumn{2}{c|}{\textbf{YouTube-UGC}} & \multicolumn{2}{c}{\textbf{\itshape Average}}  \\
		\hline
		Type & Methods & Source & SROCC & PLCC & SROCC & PLCC & SROCC & PLCC & SROCC & PLCC   \\
		\hline
		\multirow{3}{*}{Classical} & TLVQM \cite{paper8}& \footnotesize \itshape TIP, 2019 & 0.799 & 0.803  & 0.773  & 0.768  & 0.669  & 0.659 & 0.732 & 0.726 \\ 
		& VIDEVAL \cite{paper7} & \footnotesize \itshape TIP, 2021 &  0.752 & 0.751  & 0.783  & 0.780  & 0.779  & 0.773 & 0.772 & 0.772 \\ 
		& RAPIQUE \cite{paper66} & \footnotesize \itshape OJSP, 2021 &  0.755 & 0.786  & 0.803  & 0.817  & 0.759  & 0.768 & 0.774 & 0.790 \\
		\hdashline 
		\multirow{2}{*}{Classical +  Deep} & CNN+TLVQM \cite{paper67} & \footnotesize \itshape ACMMM, 2020 & 0.825 & 0.834 & 0.816 & 0.818 & 0.809 & 0.802 & 0.815 & 0.814\\
		& CNN+VIDEVAL \cite{paper7} & \footnotesize \itshape TIP, 2021 & 0.785 & 0.810 & 0.815 & 0.817 & 0.808 & 0.803 & 0.806 & 0.810\\
		\hdashline
		\multirow{6}{*}{\shortstack{Deep \\ Multi-branch}} 
		& PVQ \cite{paper16} &  \footnotesize \itshape CVPR, 2021 &  0.827 & 0.837  & 0.791  & 0.786  & NA  & NA  & NA & NA \\ 
		& BVQA \cite{paper17} & \footnotesize \itshape TCSVT, 2022 &  0.831 & 0.842  & 0.834  & 0.836  & 0.831  & 0.819 & 0.832 & 0.832 \\
		& CoINVQ \cite{paper22} & \footnotesize \itshape TCSVT, 2021 & NA & NA & 0.767 & 0.764 & 0.816 & 0.802 & NA & NA \\
		& DOVER \cite{paper64} & \footnotesize \itshape ICCV, 2023 &  0.812 & 0.852  & 0.897  &0.899  & 0.877  & 0.873 & 0.862 & 0.875\\
		& MaxVQA \cite{paper63} &\footnotesize \itshape ACMMM,2023 & 0.854 & 0.873 & 0.894 & 0.895 & \textbf{\textcolor{green!50!black}{0.894}} & \textbf{\textcolor{green!50!black}{0.890}} & 0.881 & 0.886 \\
		%		& A$^2$INet \cite{paper104}& \footnotesize \itshape ACMMM,2024 &  0.895 & 0.895  & 0.888  & 0.881  & 0.857  & 0.852  & 0.880  & 0.876 \\
		& CLiF-VQA \cite{paper80} & \footnotesize \itshape ACMMM,2024 &  \textbf{\textcolor{green!50!black}{0.866}} & 0.878  & \textbf{\textcolor{green!50!black}{0.903}}  & 0.903  & 0.888  & \textbf{\textcolor{green!50!black}{0.890}}  & \textbf{\textcolor{green!50!black}{0.886}} & \textbf{\textcolor{green!50!black}{0.890}} \\
		& MBVQA \cite{paper106} & \footnotesize \itshape CVPR, 2024 &  0.860 & \textbf{\textcolor{green!50!black}{0.880}}  & 0.901  & \textbf{\textcolor{green!50!black}{0.905}}  & 0.876  & 0.877 & 0.879 & 0.887\\
		\hdashline
		\multirow{7}{*}{\shortstack{Deep \\ Single-branch}} & VSFA \cite{paper15}& \footnotesize \itshape ACMMM, 2019 & 0.773 & 0.795 & 0.773  & 0.775  & 0.724  & 0.743 & 0.752 & 0.765 \\ 
		& GST-VQA \cite{paper41} & \footnotesize \itshape TCSVT, 2021 & NA & NA & 0.814 & 0.825 & NA & NA & NA & NA \\ 
		
		& FAST-VQA-M \cite{paper29}& \footnotesize \itshape ECCV, 2022 &  0.803 & 0.828  & 0.873  & 0.872  & 0.768  & 0.765 & 0.815 & 0.822 \\
		%	FAST-VQA \cite{paper29} & ECCV, 2022 &  0.849 & 0.865  & 0.891  & 0.892  & 0.855  & 0.852  \\
		%MaxVQA \cite{paper63} & ACMMM, 2023 & 0.854 & 0.873 & 0.894 & 0.895 & 0.894 & 0.890 & 0 & 0 \\
		& FAST-VQA \cite{paper29} & \footnotesize \itshape ECCV, 2022 &  \textbf{\textcolor{blue}{0.845}} & 0.852  & 0.890  & 0.889  &  0.857  & 0.853  & 0.864 & 0.865\\
		& FasterVQA \cite{paper19}  & \footnotesize \itshape TPAMI, 2023 &  0.843 & \textbf{\textcolor{blue}{0.858}}  & \textbf{\textcolor{blue}{0.895}}  & \textbf{\textcolor{blue}{0.898}}  & \textbf{\textcolor{blue}{0.863}}  & \textbf{\textcolor{blue}{0.859}}  & \textbf{\textcolor{blue}{0.867}} & \textbf{\textcolor{blue}{0.872}}\\
		\cline{2-11}
		& \textbf{MVQA-tiny} &  \textbf{\itshape ours} & \textbf{0.850} & \textbf{0.866} & \textbf{0.903} & \textbf{0.904} & \textbf{0.869} & \textbf{0.872} & \textbf{0.874} & \textbf{0.881} \\ 
		& \textbf{MVQA-middle} & \textbf{ \itshape ours} & \textbf{\textcolor{red}{0.878}} & \textbf{\textcolor{red}{0.895}} & \textbf{\textcolor{red}{0.925}} & \textbf{\textcolor{red}{0.925}} & \textbf{\textcolor{red}{0.901}} & \textbf{\textcolor{red}{0.903}} & \textbf{\textcolor{red}{0.901}} & \textbf{\textcolor{red}{0.908}} \\ 
		\hdashline
		\multicolumn{3}{c|}{\footnotesize \itshape improvement to existing best Single-branch}  &\footnotesize \itshape \textcolor{blue}{$3.91 \%$} &\footnotesize \itshape \textcolor{blue}{$ 4.31\%$}  &\footnotesize \itshape \textcolor{blue}{$ 3.35\%$}  &\footnotesize \itshape \textcolor{blue}{$ 3.01\%$} &\footnotesize \itshape \textcolor{blue}{$ 4.40\%$} &\footnotesize \itshape \textcolor{blue}{$ 5.12\%$} &\footnotesize \itshape \textcolor{blue}{$ 3.92\%$} &\footnotesize \itshape \textcolor{blue}{$ 4.13\%$} \\
		\hdashline
		\multicolumn{3}{c|}{\footnotesize \itshape improvement to existing best Multi-branch}  &\footnotesize \itshape \textcolor{green!50!black}{$ 1.39\% $} &\footnotesize \itshape \textcolor{green!50!black}{$ 1.71\% $}  &\footnotesize \itshape \textcolor{green!50!black}{$ 2.44\% $}  &\footnotesize \itshape \textcolor{green!50!black}{$ 2.21\% $} &\footnotesize \itshape \textcolor{green!50!black}{$ 0.78\% $} &\footnotesize \itshape \textcolor{green!50!black}{$ 1.46\% $} &\footnotesize \itshape \textcolor{green!50!black}{$ 1.69\% $} &\footnotesize \itshape \textcolor{green!50!black}{$ 2.02\% $} \\
		\bottomrule
	\end{tabular}
	\vspace{-0.4cm}
\end{table*}

\subsection{Experiment Results}


\textbf{Pre-training Results on LSVQ.}
We pre-train the proposed MVQA on LSVQ and conduct intra-dataset testing on LSVQ$_{test}$ and LSVQ$_{1080p}$. Additionally, cross-dataset testing was performed on KoNViD-1k and LIVE-VQC. 
The results are shown in \cref{table1}.
First, for our tiny version of the MVQA model, compared to the current best-performing and fastest FasterVQA model, our model achieves comparable performance while offering faster processing speed.
In addition, for the middle version of MVQA, compared with the classical methods  (BRISQUE, TLVQM, VIDEVAL), our method shows superior performance on all test sets. Our model also achieves better results compared to deep learning-based methods. 
Specifically, compared to the current state-of-the-art single-branch models, our model achieve average improvements of $4.02 \%$ and $ 3.59 \%$ in SROCC and PLCC metrics for intra-dataset testing. In cross-dataset testing, the improvements are $2.92 \%$ and $ 3.29 \%$, respectively.
Since single-branch models often struggle to simultaneously capture both quality and semantic features of videos, recent multi-branch models, which better incorporate video semantic information, have shown outstanding performance.
The performance of our single-branch based MVQA model is still ahead of all current multi-branch models.
Compared to the current state-of-the-art results, our model achieves improvements of $0.92 \%$  and $ 0.79 \%$ in SROCC and PLCC, respectively, while offering higher computational efficiency.


\noindent
\textbf{Fine-tuning Results on Small Datasets.}
\begin{table}[h]
	%	\vspace{-0.2cm}
	\setlength{\abovecaptionskip}{0.01cm}
	\caption{FLOPs and running time(average of 10 runs) on GPU (RTX 3090). FLOPs and time are in $G$ and $s$, respectively.}
	\centering
	\footnotesize
	\setlength\tabcolsep{3.9pt}  %列间距
	%\setlength{\baselineskip}{50pt} %行间距
	%	\setlength{\baselineskip}{5\baselineskip}
	\renewcommand\arraystretch{1}
	
	\setlength{\aboverulesep}{0pt}
	\setlength{\belowrulesep}{0pt}
	\begin{tabular}{l|c:c|c:c|c:c}
		\toprule
		\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{\textbf{540p}} & \multicolumn{2}{c|}{\textbf{720p}} & \multicolumn{2}{c}{\textbf{1080p}} \\
		\cline{ 2 - 7}
		&FLOPs & Time &  FLOPs & Time &FLOPs & Time  \\
		\hline
		VSFA \cite{paper15} & 6440 & 1.506  & 11426 & 2.556 & 25712 & 5.291\\
		PVQ \cite{paper16} & 9203 &1.792&13842&2.968&36760&6.556\\
		BVQA \cite{paper17} &17705 &3.145&31533&7.813&70714 &14.34\\
		FAST-VQA \cite{paper29} & 284 &0.056&284&0.056 &284&0.056\\
		FasterVQA \cite{paper19} & 70  & 0.032  & 70 & 0.032 & 70  & 0.032 \\
		%		Faster-VQA \cite{paper19} & 71 &&&71&&&71&&\\
		DOVER \cite{paper64} &282 &0.061&282&0.061&282&0.062 \\
		CLiF-VQA \cite{paper80} & 1432 &0.522&1432&0.522&1432&0.522\\
		MBVQA \cite{paper106} & 912 & 0.194 & 1232 & 0.267 & 2150 & 0.891 \\
		\hline
		\textbf{MVQA-tiny} & \textbf{34} & \textbf{0.028}& \textbf{34} & \textbf{0.028} &\textbf{34} &\textbf{0.028}\\
		\textbf{MVQA-middle} &\textbf{ 403} & \textbf{0.130} &\textbf{ 403} & \textbf{0.130} & \textbf{403} & \textbf{0.130} \\
		\bottomrule
	\end{tabular}
	\label{table3}
	\vspace{-0.4cm}
\end{table}
We fine-tune MVQA on three small datasets (LIVE-VQC, KoNViD-1k, YouTube-UGC), as shown in \cref{table2}.
We can see that MVQA-tiny achieves comparable performance compared to the current best single-branch model.
Moreover, MVQA-middle achieves improvements of $3.92 \%$ and $4.13 \%$ in SROCC and PLCC, respectively, on three datasets compared to the best results from single-branch models.
Additionally, compared to the best multi-branch models, it shows improvements of  $1.69 \%$ and  $2.02 \%$ in SROCC and PLCC, respectively.

%\begin{figure*}[h]
%	\vspace{-0.4cm}
%	\centering
%	\setlength{\abovecaptionskip}{0.1cm}
%	\includegraphics[scale=0.13]{img//4.3.png}
%	\caption{A schematic of the different scale masks. We perform mask fusion between distortion sampling and semantic sampling at different proportions, embedding the smaller sampling results into the larger ones. The red boxes represent the embedding locations.}
%	\label{fig4.3}
%	\vspace{-0.4cm}
%\end{figure*}


\subsection{Efficiency}
To test the efficiency, we compare MVQA with the current mainstream deep learning-based models.
Specifically, we compare the FLOPs and GPU runtimes for videos of different resolutions, where the length of the videos are 150 frames, as shown in \cref{table3}.
Compared to CNN-based models (VSFA, PVQ, BVQA), MVQA-tiny reduces FLOPs by up to $756\times$, $1081\times$, and $2079\times$, as well as reduces computation time by up to $189\times$, $234\times$, and $512\times$, respectively.
%Moreover, our model achieves a $8.35\times$ reduction in FLOPS and a $2\times$ reduction in computation time compared to FAST-VQA.
Moreover, compared to the fastest FasterVQA, our model has comparable computational computation as well as a $2\times $ reduction in flops.
In addition, MVQA-middle not only performs better but also reduce FLOPs by up to $3.55\times $ and $5.33 \times$, and computation time by up to $ 4.02\times$ and $6.85 \times$, respectively, compared to the current best models CLiF-VQA and MBVQA.

\begin{table}[t]
	\vspace{-0.4cm}
	\setlength{\abovecaptionskip}{0.01cm}
	\caption{USDS performance in the  Video Swin Transformer.}
	\centering\setlength{\tabcolsep}{3.1pt}
	\label{table12}
	\footnotesize
	\setlength{\aboverulesep}{0pt}
	\setlength{\belowrulesep}{0pt}
	\begin{tabular}{l|cc|cc|cc}
		\toprule
		Datasets &\multicolumn{2}{c|}{\textbf{LSVQ$_{test}$}} & \multicolumn{2}{c|}{\textbf{KoNViD-1k}} & \multicolumn{2}{c}{\textbf{LIVE-VQC}}   \\
		\hline
		Sampling & SROCC & PLCC & SROCC & PLCC & SROCC & PLCC  \\
		\hline
		\itshape Fragments & 0.872 & 0.874 & 0.864 & 0.862 & 0.824 & 0.841 \\
		\textbf{USDS} & \textcolor{red}{0.877} & \textcolor{red}{0.879} & \textcolor{red}{0.871} & \textcolor{red}{0.869} & \textcolor{red}{0.832} & \textcolor{red}{0.851} \\
		\bottomrule
	\end{tabular}
%	\vspace{-0.2cm}
\end{table}


\subsection{Evaluation on USDS}

\begin{figure}[t]
	\vspace{-0.2cm}
	\centering
	\setlength{\abovecaptionskip}{0.1cm}
	\includegraphics[scale=0.3]{5.png}
	\caption{Results of semantic analysis experiments.}
	\label{qualitative analysis}
	\vspace{-0.4cm}
\end{figure}

\noindent
\textbf{Semantic Analysis.}
We conduct experiments to verify that USDS can capture sufficient semantic information.
%In order to verify that USDS can capture sufficient semantic information, we conduct qualitative experiments.
Consistent with the testing method in Fig. \ref{fig1.5}, 
we use CLIP model with strong visual language capabilities to validate the semantic information in the sampled maps.
As shown in Fig. \ref{qualitative analysis}, USDS can retain more semantics compared to Fragments.
More qualitative results can be found in the Appendix.

%In addition, we conduct experiments to further illustrate that USDS can retain semantics well.


%we conduct qualitative (as shown in Fig. \ref{qualitative analysis}) and quantitative experiments (Table 7) separately. 


\noindent
\textbf{Cross-Architecture Validation.}
To demonstrate the advantages of USDS under different models.
We validate USDS's effectiveness in the Video Swin Transformer, the dominant architecture in VQA, as shown in Tab. \ref{table12}.
The results show that USDS is not only effective in the proposed MVQA architecture, but also in the Video Swin Transformer model due to the traditional Fragments sampling method.

\subsection{Ablation Studies}


%\begin{table}[h]
%	\setlength{\abovecaptionskip}{0.1cm}
%	\caption{Ablation study on proportion of semantic information.}
%	\centering\setlength{\tabcolsep}{4pt}
%	\label{table5}
%	\footnotesize
%	\setlength{\aboverulesep}{0pt}
%	\setlength{\belowrulesep}{0pt}
%	\begin{tabular}{l|cc|cc|cc}
	%		\toprule
	%		Datasets &\multicolumn{2}{c|}{\textbf{LSVQ$_{test}$}} & \multicolumn{2}{c|}{\textbf{KoNViD-1k}} & \multicolumn{2}{c}{\textbf{LIVE-VQC}}   \\
	%		\hline
	%		Proportion & SROCC & PLCC & SROCC & PLCC & SROCC & PLCC  \\
	%		\hline
	%		$1/16$ & 0.834 & 0.830 & 0.826 & 0.824 & 0.760 & 0.795  \\
	%		$15/16$ & 0.820 & 0.815 & 0.811 & 0.815 & 0.749 & 0.780  \\
	%		$2/4$ & 0.865 &0.866 & 0.857 & 0.861 & 0.795 & 0.838  \\
	%		$3/4$ & 0.856 & 0.859 & 0.830 & 0.836& 0.772 & 0.820 \\
	%		\hdashline
	%		$1/4$ & \textcolor{red}{0.874} & \textcolor{red}{0.874} & \textcolor{red}{0.865} & \textcolor{red}{0.867} & \textcolor{red}{0.800} & \textcolor{red}{0.847} \\
	%		\bottomrule
	%	\end{tabular}
%	\vspace{-0.4cm}
%\end{table}

\noindent
\textbf{Ablation on Sampling.} 
We compare the proposed USDS with four common sampling methods (resize, crop, MRET \cite{paper102}, fragments \cite{paper29}) to validate its effectiveness. 
To ensure a fair comparison, we keep the model structure and the block size used for frame segmentation during input unchanged. As shown in \cref{table4}.
Specifically, USDS performs very well compared to traditional resize and crop sampling.
Additionally, compared to the currently most effective sampling method, fragments , which can fully and evenly preserve the local texture of the video, USDS shows improvements of $2.99 \%$ and $2.00 \%$ in SROCC and PLCC, respectively. This demonstrates that USDS not only preserves the local texture of the video to the greatest extent but also retains more semantic information.

\begin{table}[t]
	\vspace{-0.4cm}
	\setlength{\abovecaptionskip}{0.01cm}
	\caption{Ablation study on different sampling methods in MVQA.}
	\centering\setlength{\tabcolsep}{3.3pt}
	\label{table4}
	\footnotesize
	\setlength{\aboverulesep}{0pt}
	\setlength{\belowrulesep}{0pt}
	\begin{tabular}{l|cc|cc|cc}
		\toprule
		Datasets &\multicolumn{2}{c|}{\textbf{LSVQ$_{test}$}} & \multicolumn{2}{c|}{\textbf{KoNViD-1k}} & \multicolumn{2}{c}{\textbf{LIVE-VQC}}   \\
		\hline
		Sampling & SROCC & PLCC & SROCC & PLCC & SROCC & PLCC  \\
		\hline
		\itshape Resize & 0.847 & 0.851 & 0.834 & 0.836 & 0.762 & 0.809  \\
		\itshape Crop & 0.798 & 0.810 & 0.765 & 0.779 & 0.744 & 0.762  \\
		\itshape MRET \cite{paper102} & 0.851 &0.854 & 0.841 & 0.839 & 0.785 & 0.820  \\
		\itshape Fragments \cite{paper29} & 0.864 & 0.865 & 0.850 & 0.853& 0.791 & 0.829 \\
		\hdashline
		\textbf{USDS} & \textcolor{red}{0.882} & \textcolor{red}{0.883} & \textcolor{red}{0.870} & \textcolor{red}{0.868} & \textcolor{red}{0.828} & \textcolor{red}{0.848} \\
		\bottomrule
	\end{tabular}
	\vspace{-0.2cm}
\end{table}
%\noindent
%\textbf{Ablation on Proportion of Mask.}
%During the sampling masking process, we can set the masking ratio to determine the amount of semantic content to be retained, as shown in \cref{fig4.3}. The experimental results with different mask ratios are shown in \cref{table5}.
%When masking at ratios of $1/16$ and $15/16$, the size of the sampled blocks is $8\times 8$. However, since the input block size of the model is $16\times 16$, each input block contains four smaller blocks. This leads to ineffective extraction of feature information from each smaller block by the 3D patch embedding, resulting in poorer performance. 
%Additionally, when the ratio is set to $1/2$ and $3/4$, the performance decreases, which suggests that while semantic information plays an important role in VQA, quality information has a greater impact on quality assessment.

\begin{figure}[t]
	\centering
	\setlength{\abovecaptionskip}{0.1cm}
	%	\setlength{\belowcaptionskip}{-0.1cm}
	%	
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{4.1.png}
		\centerline{ \footnotesize (a) PLCC}
	\end{minipage}
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{4.2.png}
		\centerline{\footnotesize (b) SROCC}
	\end{minipage}
	\caption{Ablation study on different resolutions. }
	\label{fig6}
	\vspace{-0.4cm}
\end{figure}

\noindent
\textbf{Ablation on Different Resolutions.} 
To further validate the effectiveness of the semantic information extracted by USDS, we conducted ablation experiments at different video resolutions. Since both MRET \cite{paper102} and Fragments \cite{paper29} sample fixed-size blocks from the video, at higher video resolutions, the sampling results become highly fragmented, often leading to a complete loss of semantic information.
As shown in \cref{fig6}.
Since the MRET sampling strategy performs multi-scale sampling from four regions of the video, when the video resolution is too high, it can only sample from localized areas of the video. This results in the sampling not fully capturing the quality information of the video.
Although the Fragments sampling method can sample uniformly from the video, at high resolutions, the features sampled using this method completely lose semantic information.
The experimental results show that as the resolution increases, the advantages of USDS become more pronounced. This is because we have effectively embedded the semantic information during the sampling process.


==> ICCV2025-Author-Kit-Feb/5_conclusion.tex <==
\section{Conclusion}
%In this paper, we are the first to explore the role of recent state space models (mamba) in VQA, aiming to address the trade-off between efficient computation and excellent performance.
%First, we propose an effective sampling method, USDS, which can efficiently integrate video semantic information, and introduce MVQA, a VQA model entirely based on state-space models (SSM). 
%Extensive experiments across multiple datasets demonstrate that MVQA is a simple, effective, and highly efficient VQA model.
In this paper, we are the first to explore the application of recent state-space models (Mamba) in VQA, aiming to balance computational efficiency with excellent performance. We first propose an effective sampling method, USDS, which efficiently integrates video semantic information, and introduce MVQA, a VQA model entirely based on state-space models (SSM). Extensive experiments across multiple datasets demonstrate that MVQA is a simple, effective, and highly efficient VQA model.






==> ICCV2025-Author-Kit-Feb/preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


